Low Rank Factorization for Compact Multi-Head Self-Attention

Effective representation learning from text has been an active area of research in the fields of NLP and text mining. Attention mechanisms have been at the forefront in order to learn contextual sentence representations. Current state-of-the-art approaches for many NLP tasks use large pre-trained language models such as BERT, XLNet and so on for learning representations. These models are based on the Transformer architecture that involves recurrent blocks of computation consisting of multi-head self-attention and feedforward networks. One of the major bottlenecks largely contributing to the computational complexity of the Transformer models is the self-attention layer, that is both computationally expensive and parameter intensive. In this work, we introduce a novel multi-head self-attention mechanism operating on GRUs that is shown to be computationally cheaper and more parameter efficient than self-attention mechanism proposed in Transformers for text classification tasks. The efficiency of our approach mainly stems from two optimizations; 1) we use low-rank matrix factorization of the affinity matrix to efficiently get multiple attention distributions instead of having separate parameters for each head 2) attention scores are obtained by querying a global context vector instead of densely querying all the words in the sentence. We evaluate the performance of the proposed model on tasks such as sentiment analysis from movie reviews, predicting business ratings from reviews and classifying news articles into topics. We find that the proposed approach matches or outperforms a series of strong baselines and is more parameter efficient than comparable multi-head approaches. We also perform qualitative analyses to verify that the proposed approach is interpretable and captures context-dependent word importance.

==> CIKM 2020/sections/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
In this paper we presented a novel compact multi-head attention mechanism and illustrated its effectiveness on text classification benchmarks. The proposed method computes multiple attention distributions over words which leads to contextual sentence representations.
The results showed that this mechanism performed better than several other approaches with fewer parameters. We also verified that the model captured context-dependent word importance. 
% including non-contextual unsupervised baselines such as average of word embeddings, contextual baselines such as RNN-based methods and CNNs and also  other attention mechanisms with fewer parameters. 
We envision two directions for future work -- 1) Currently, the model relies on RNNs that makes it slower due to their sequential computation. We seek to investigate ways of adapting the proposed mechanism in Transformer-style self-supervised language models such as BERT, XLNet etc. without dependency on RNNs by incorporating positional embeddings ~\citep{GehringConvS2S} for faster and efficient learning of language representations; 2) currently, the model uses a single global context vector as the query vector that conflates the entire sentence into one vector which could lead to information loss. Transformer models on the other hand use fine-grained context by querying every word in the sequence for each candidate word. Even though this may help develop direct connections between relevant words it might get redundant. In the future work, we seek to investigate ways of incorporating phrase-level queries as a middle ground between a single global context vector like the proposed approach and fine-grained queries like Transformer providing a balance between complexity and context.
% The compactness of the proposed model will bring in more computational savings in cases where multiple multi-head attention mechanisms are used example transformer models in neural machine translation. We leave this as future work.
% An important research question concerns with the discernibility of different attention heads with respect to each other for better interpretablity. One of the obstacles in learning attention in an unsupervised way is that there is no implicit mechanism to impose structure on different rows; although it merits further research. 






% Also the current model is heavily dependent on the downstream tasks and thus learning transferable representations is hard. Although we can still do unsupervised learning on the proposed model by using a sequential decoder on top of the sentence embedding, it merits more to find some other structures as a decoder.

==> CIKM 2020/sections/intro.tex <==
\section{Introduction}
% \textcolor{Huzefa}{What is the big problem here that needs these representations }

%  Learning effective language representations is important for a variety of text analysis tasks including sentiment analysis, news classification, natural language inference and question answering. Previous approaches to learning such representations were limited to learning distributed word representations also known as word embeddings ~\citep{bengio2003neural,collobert2011natural,mikolov2013distributed,Pennington2014GloveGV}. Sentence embeddings were composed by aggregating the individual word embeddings and this approach indeed forms a strong baseline ~\citep{Arora2017ASB}. These representations however are not contextual and  can be improved by capturing semantics at the sentence level. 
% % Researchers have tried to replicate the success of word embeddings to capturing representations of sentences and their meaning. 
% % Words being a more granular and naturally transferable unit of representation across different tasks and languages, there's a consensus regarding usefulness of word embeddings and the meaning of their representations (e.g. semantic correlatedness) and how to learn them. However, it is not yet clear and even harder to capture general purpose transferable representations in a fixed sized vector.
% % Sentence embedding methods fall in two categories: (i) consisting of universal sentence embeddings usually trained by unsupervised methods ~\citep{hill2016learning} including SkipThought, QuickThought ~\citep{Kiros:2015:SV:2969442.2969607,logeswaran2018an}, ParagraphVector ~\citep{le2014distributed} etc. (ii) Supervised approaches that learn general purpose sentence representations by training a large corpus of data over multiple tasks ~\citep{conneau2017supervised}. Infersent learns transferable sentence representations by training a rather simple model on the Stanford Natural Language Inference Task (SNLI) ~\citep{bowman2015large}. It leverages a single task albeit a meaningful one to learn the representations. 
% Although there are efforts to improve sentence representations using the above paradigms, in practice the best performing models are narrow experts as opposed to broad generalists and use sentence embeddings as an intermediate step in models that are specifically  trained for one task by supervised learning.

%To learn more generalizable sentence embeddings researchers have used multi-task learning 

% Multi-task learning approaches have incorporated 
% data from diverse sources within the learning models.  Subramanium et al. ~\citep{subramanian2018learning} use multi-task learning to train a single encoder-decoder model on six distinct tasks. Universal Sentence Encoder ~\citep{cer2018universal} follows a similar approach by using a Transformer ~\citep{vaswani2017attention} model instead. Generalizing on a wide variety of downstream tasks to capture various syntactic and semantic properties of text is a hard problem and gains are observed only for a few tasks. 
% \textcolor{Huzefa}{I miss context why this para is here and what's going on}

% \begin{figure}

%  \centering
% \colorbox{MyBlue!38.5991}{atmosphere} \colorbox{MyBlue!10.7567}{was} \colorbox{MyBlue!80.9065}{great}
% \colorbox{MyBlue!10.2716}{.}
% \colorbox{MyBlue!10.2716}{the} \colorbox{MyBlue!100.3384}{octopus} \colorbox{MyBlue!10.4075}{was} \colorbox{MyBlue!98.6137}{delicious}  \colorbox{MyBlue!10.5932}{with} \colorbox{MyBlue!10.9595}{the} \colorbox{MyBlue!100.9002}{balsamic} \colorbox{MyBlue!101.0958}{reduction} \colorbox{MyBlue!10.469}{as} \colorbox{MyBlue!10.5344}{a} \colorbox{MyBlue!95.3144}{nice} \colorbox{MyBlue!98.9393}{touch} \colorbox{MyBlue!10.2716}{.} \colorbox{MyBlue!35.7487}{have} \colorbox{MyBlue!35.7461}{a} \colorbox{MyBlue!36.7514}{nice} \colorbox{MyBlue!37.0122}{lunch} \\
% \caption{An example review from the Yelp dataset. A visualization of the  important words attended by our model and how it helps classify the review as having a rating of 5.}
%   \label{fig:exvis2}
% \end{figure}

%  Several approaches model sequential dependencies in the text by using recurrent neural networks ~\citep{hochreiter1997long}; recursive networks ~\citep{socher2013recursive} and convolutional networks ~\citep{DBLP:conf/ijcnlp/ZhangW17,kim2014convolutional}  to solve classification and ranking problems.  These approces usually  create a simple vector representation by using the final hidden state of the RNN or the max (or average) pooling from either RNN hidden states or convolved n-grams ~\citep{kim2014convolutional}. RNNs, even LSTMs suffer from long term dependency issue due to the vanishing gradient problem ~\citep{Hochreiter:1997:LSM:1246443.1246450} and fail to carry the semantics along all time steps of a recurrent model.

%is relatively hard. 
Learning effective language representation is important for a variety of text analysis tasks including sentiment analysis, news classification, natural language inference and question answering. 
% Language representations can be learned via supervised, self-supervised approaches.
Supervised learning using neural networks commonly entails learning intermediate sentence representations followed by a task specific layer. For text classification tasks; this is usually a fully connected layer followed by an \textit{N-way} softmax where \textit{N} is the number of classes. 

Learning self-supervised language representations has made substantial progress in recent years with the introduction of new techniques for language modeling  combined with deep models like ELMo~\citep{peters2018deep}, ULMFit ~\citep{howard2018universal} and more recently BERT ~\citep{devlin2018bert} and GPT-2 ~\citep{radford2019language}. There has been a surge of BERT-based language models that use larger data for pretraining and different pretraining methods such as XL-Net ~\citep{yang2019xlnet}, RoBERTa ~\citep{liu2019roberta} while others combine different modalities ~\citep{su2019vl}. These methods have enabled transfer of learned representations via pre-training to downstream tasks.
% Recently, the BERT model which uses a modification of the language modeling task and uses unlabeled data for pretraining the transformer model ~\citep{vaswani2017attention} has shown improvements on a variety of NLP tasks ~\citep{devlin2018bert}. 
Although these models work well on a variety of tasks there are two major limitations: 1) they are  computationally expensive to train 2) they usually have a large number of parameters that greatly increases the model size and memory requirements. For instance, the multilingual BERT-base cased model has 110M parameters, the small GPT-2 model has 117M parameters ~\citep{radford2019language} and the RoBERTa model was trained on 160GB of data ~\citep{liu2019roberta}. Recently, researchers have proposed `lighter' BERT models that leverage knowledge distillation during the pre-training phase and reduce the size of the BERT model ~\citep{wolf2019transformers} or  try to improve the parameter efficiency of the BERT model by optimizations at the embedding layer and by parameter sharing ~\citep{lan2019albert}. However, all of the above models are based on the Transformer architecture ~\citep{vaswani2017attention} the major component of which is the scaled dot-product self-attention mechanism .   
% It is natural to see how task specific training (ELMo) or fine-tuning (BERT, GPT-2) can be limiting when the  training data and computational resources are scarce. 
% Further, running inference on and storing such models can also be difficult in low resource scenarios such as IoT devices or low-latency use cases. Hence, supervised learning for task-specific architectures which are trained from scratch, especially where domain specific training data is available are useful. They are light-weight and easy to deploy. In this work we focus on learning compact attention-based supervised language representations with text classification as the downstream task. 

% Modern neural networks have a large number of parameters. Computation at attention layers in these networks can get prohibitive. Especially, multi-head attention mechanisms including \textit{luong-style} mechanisms  ~\citep{lin2017structured,guo2017end} and Transformer-based mechanims ~\citep{vaswani2017attention} 
% % (multiple attention distributions over a given sentence)
% that form an integral part of many state-of-the-art architectures for NLP tasks ~\citep{vaswani2017attention,devlin2018bert} can be expensive to compute.
This layer has a computational complexity of $O(n^2*d)$ that scales quadratically with the length of the input ($n$) and linearly with the length of the model hidden size ($d)$.
% We argue that this layer giving rise to multiple attentions in the Transformer architecture is over-parameterized.
It is natural to see how task specific training or fine-tuning can be limiting when the  training data and computational resources are scarce and sequences are long. 
Further, running inference on and storing such models can also be difficult in low resource scenarios such as IoT devices or low-latency use cases. Hence, supervised learning for task-specific architectures which are trained from scratch, especially where domain specific training data is available are useful. They are light-weight and easy to deploy. In this work, we propose \textbf{l}ow-rank f\textbf{a}ctorization based \textbf{m}ulti-head \textbf{a}ttention mechanism (LAMA), a lean attention mechanism which is computationally cheaper and more parameter efficient than prior approaches and exceeds or matches the performance of state-of-the-art baselines including large pretrained models, with fewer parameters.
%  Several approaches learn supervised sentence representations by using recurrent neural networks (RNN) augmented with attention mechanisms ~\citep{han,lin2017structured}. Attention mechanisms alleviate the vanishing gradient problem by giving direct access to RNN hidden states to compute sentence representations. However these attention mechanisms either capture only a single aspect of the meaning of a sentence ~\citep{han} or capture multiple aspects by replicating the parameters followed by a simple  concatenation operation on the learned representations ~\citep{conneau2017word,guo2017end}. Lin et al. ~\citep{lin2017structured} proposed an approach in which multiple attention distributions are obtained from a single set of parameters, but attention is concentrated on individual words missing out on phrase level (bi-gram, tri-gram etc.) context. 
%   To address these issues, we propose a novel attention mechanism, which is used to construct a structured sentence embedding. Our method  1) captures nuanced context by assigning similar attention weights to frequently co-occurring words.
% 2) captures multiple attention distributions to build a rich contextual embedding.
 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[!ht]
% \caption{}
% \begin{tabular}{@{}ll@{}}
% \colorbox{MyPurple!20.84}{restaurant} \colorbox{MyPurple!0.33}{was} \colorbox{MyPurple!0.099116}{overall} \colorbox{MyPurple!83.9}{good} \colorbox{MyPurple!2.3}{but} \colorbox{MyPurple!3.4743}{not} \colorbox{MyPurple!0.07201}{great} & Predicted=2 \\
% \colorbox{MyPurple!24.0}{restaurant} \colorbox{MyPurple!10.0}{was} \colorbox{MyPurple!36.0}{overall} \colorbox{MyPurple!65.0}{good} \colorbox{MyPurple!63.0}{but} \colorbox{MyPurple!63.0}{not} \colorbox{MyPurple!37.0}{great} & \\
% \end{tabular}
% \end{table}

% The effectiveness and efficiency of our approach comes from two factors: 1)
Contrary to previous approaches ~\citep{lin2017structured,guo2017end} that are based on additive attention mechanism ~\citep{neuralAlign}, LAMA is based on multiplicative attention ~\citep{luong2015effective} which replaced the additive attention by dot product for faster computation. We further introduce a bilinear projection while computing the dot product to capture similarities between a global context vector and each word in the sentence ~\citep{luong2015effective}. The function of the bilinear projection is to capture nuanced context dependent word-importance as corroborated by previous works ~\citep{chen2017reading}. Next, unlike previous methods we use low-rank formulation of the bilinear projection matrix based on hadarmard product ~\citep{kim2016hadamard,yu2015combining}
% This has previously proven to be effective in capturing similarity between a context paragraph and a query in question answering (unimodal) \citep{chen2017reading} and image features and query in visual question answering (multimodal) (VQA) ~\citep{kim2014convolutional} 
% Specifically we use hadarmard product for low-rank factorized bilinear pooling ~\citep{kim2016hadamard,yu2017multi} . 
% This approach uses matrix factorization for a fast approximation of the outer product of features in two high-dimensional feature spaces to give a lower dimensional output ~\citep{kim2016hadamard}.
to produce multiple attentions by querying the global context vector for each word as opposed to having a different learned vector ~\citep{lin2017structured} or matrix ~\citep{yu2017multi}. In effect, we cast score computation between a word representation and a context vector as unimodal feature fusion to a low dimensional space akin to its multimodal counterparts ~\citep{yu2017multi,lin2015bilinear}. Each dimension of this low-dimensional feature space can be considered as the contribution of the word to a different attention head. By controlling the dimension of this feature space new heads can be added or removed. Finally, we devise a mechanism to obtain context-aware supervised sentence embeddings from the obtained attention distributions for downstream classification tasks. We evaluate our model on tasks such as sentiment analysis, predicting business ratings and news classification. We show that the proposed model learns context-dependent word importance like other attention models. Moreover, the proposed model is 3 times more parameter efficient than other comparable attention models especially the encoder of a Transformer model ~\citep{vaswani2017attention}. In terms of performance, the proposed model is competitive and matches or exceeds the performance of strong baselines, attention and non-attention based. Further, we present some ancillary analyses on model efficiency and need for multiple attention heads. In summary, our results show that the proposed model can be reliably used as a leaner multi-head attention alternative for supervised text classification tasks.

The organization of the rest of the paper is as follows: the next section (\S\ref{sec:rw}) discusses connections with related work, followed by the description of the proposed model (\S\ref{sec:model}), followed by the task descriptions and  the experimental evaluation (\S\ref{sec:experiments}). Finally, in the following sections the results are presented along with their discussion (\S\ref{sec:results}), before concluding (\S\ref{sec:conclusion}). 

% To summarize, our contributions can be succinctly described as follows:
% \begin{itemize}[leftmargin=0cm,itemindent=0.3cm,labelwidth=\itemindent,labelsep=0cm,align=left,nosep]
%     \item We propose a low-rank formulation for computing multi-aspect attention to form a compact sentence representation.
%     %than previous approaches.
%     \item Our embedding can be constructed by using as many as 70 times fewer parameters than previous approaches while outperforming them in terms of downstream classification tasks.
%     % \item We will make our code publicly available 
% \end{itemize}

% The proposed attention method uses a bilinear projection to capture similarities between a global context vector and each word in the sentence. We find that using bilinear projection is instrumental in learning phrase-level context. This has previously proven to be effective in capturing similarity between a context paragraph and a query in question answering (unimodal) \citep{chen2017reading} and image features and query in visual question answering (multimodal) (VQA) ~\citep{kim2014convolutional} 

% To construct a structured embedding we compute multiple attentions over the sentence. Unlike previous approaches, to efficiently compute multiple attentions we use low-rank factorized bilinear pooling ~\citep{yu2017multi}. 
% % This approach uses matrix factorization for a fast approximation of the outer product of features in two high-dimensional feature spaces to give a lower dimensional output ~\citep{kim2016hadamard}.
% This approach uses matrix factorization to decompose a single bilinear matrix to produce multiple attentions between the global context vector and each word.
% We evaluate our model by performing experiments on multiple datasets spanning two different tasks namely Sentiment Analysis and Text Classification. We find that our model outperforms a set of strong baselines at a much lower computational cost.
% To summarize, our contributions can be succinctly described as follows:
% \begin{itemize}[leftmargin=0cm,itemindent=0.3cm,labelwidth=\itemindent,labelsep=0cm,align=left,nosep]
%     \item We present an efficient novel attention mechanism by fusing sentence level context and word level features to construct a structured sentence embedding.
%     %than previous approaches.
%     \item Our embedding can be constructed by using as many as 70 times fewer parameters than previous approaches while outperforming them.
% \end{itemize}

==> CIKM 2020/sections/methods.tex <==
\section{Proposed Model} \label{sec:model}
In this section, we give an overview of the proposed model followed by a detailed description of each model component.

A document (a product review or a news article) is first tokenized and converted to a word embedding via a lookup into a pretrained embedding matrix. The embedding of each token is encoded via a bi-directional Gated Recurrent Unit ~\citep{cho2014learning} (bi-GRU) sentence encoder to get a contextual annotation of each word in that document. The LAMA attention mechanism then obtains multiple attention distributions over those words by computing an alignment score of their hidden representation with a word-level context vector. Sum of the word representations weighted by the scores from multiple attention distributions then forms a matrix document embedding. The matrix embedding is then flattened and passed onto downstream layers (either a classifier or another encoder depending on the task). 

In the rest of the paper, capital bold letters indicate matrices, small bold letters indicate vectors and small letters indicate scalars.
 
%  In the following sections we describe the propsed embedding in detail. Matrices are denoted by bold capital letters, vectors by bold small letters and unbolded small letters are scalars. Please use table ~\ref{tab:note} to cross-reference the important notations.
 
\subsection{Sequence Encoder}
 We use the GRU ~\citep{neuralAlign} RNN as the sequence encoder. GRU uses a gating mechanism to track the state of the sequences. There are two types of gates: the reset gate $\textbf{r}_t$ and the update gate $\textbf{z}_t$. The update gate decides how much past information is kept and how much new information is added.  At time $t$, the GRU computes its new state as:
\begin{align}
 \textbf{h}_t = (1-\textbf{z}_t) \odot \textbf{h}_{t-1} + \textbf{z}_t  \odot \Tilde{\textbf{h}}
\end{align}
and the update gate $\textbf{z}_t$ is updated as:
 \begin{align}
   \textbf{z}_t = \sigma(\textbf{W}_z*\textbf{x}_t + \textbf{U}_z*\textbf{h}_{t-1} + \textbf{b}_z)   
 \end{align}
The RNN candidate state $\Tilde{\textbf{h}_t}$ is computed as:
\begin{align}
\Tilde{\textbf{h}_t} = tanh(\textbf{W}_h\textbf{x}_t + \textbf{r}_t \odot (\textbf{U}_h \textbf{h}_{t-1} + \textbf{b}_h)
\end{align}
Here $\textbf{r}_t$ is the reset gate which controls how much the past state contributes to the candidate state. If $\textbf{r}_t$ is zero, then it forgets the previous state. The reset gate is updated as follows:
\begin{align}
\textbf{r}_t = \sigma(\textbf{W}_r\textbf{x}_t + \textbf{U}_r\textbf{h}_{t-1} + \textbf{b}_r)
\end{align}
Consider a document $D_i$ containing $T$ words. $D_i=\{\textbf{w}_{1},...,\textbf{w}_{t},...,\textbf{w}_{T}\}$. Let each word be denoted by $\textbf{w}_{t}$, $t \in [0, T]$  where every word is converted to a real valued word vector $\textbf{x}_{t}$ using a pre-trained embedding matrix $\textbf{W}_e = R^{d \times |V|}$, $\textbf{x}_{t} = \textbf{W}_e \textbf{w}_{t}$, $t \in [1, T]$  where $d$ is the embedding dimension and $V$ is the vocabulary. The embedding matrix $\textbf{W}_e$ is fine-tuned during training. Note that we have dropped the subscript $i$ as all the derivations are for the $i^{th}$ document and it is assumed implicit in the following sections unless otherwise stated.

We encode the document using a bi-GRU that summarizes information in both directions along the text to get a contextual annotation of a word. In a bi-GRU the hidden state at time step $t$ is represented as a concatenation of hidden states in the forward and backward direction. The forward GRU denoted by $\overrightarrow{GRU}$ processes the document from $w_{1}$ to $w_{T}$ whereas the backward GRU denoted by $\overleftarrow{GRU}$ processes it from $w_{T}$ to $w_{1}$.


\begin{align}
\textbf{x}_{t} = \textbf{W}_e \textbf{w}_{t}
\end{align}
\begin{subequations}
\begin{align}
\overrightarrow{\textbf{h}_{t}} = \overrightarrow{GRU}(\textbf{x}_{t}, \textbf{h}_{(t-1)}, \mbox{\boldmath$\theta$})
\end{align}
\begin{align}
\overleftarrow{\textbf{h}_{t}} = \overleftarrow{GRU}(\textbf{x}_{t}, \textbf{h}_{(t+1)}, \mbox{\boldmath$\theta$})
\end{align}
\end{subequations}
Here the word annotation $\textbf{h}_{t}$ is obtained by concatenating the forward hidden state $\overrightarrow{\textbf{h}_{t}}$ and the backward hidden state $\overleftarrow{\textbf{h}_{t}}$.

\subsection{Single-Head Attention}
To alleviate the burden of remembering long term dependencies from GRUs we use the global attention mechanism ~\citep{luong2015effective} in which the document representation is computed by attending to all words in the document. Let $\textbf{h}_{t}$ be the annotation corresponding to the word $\textbf{x}_{t}$. First we transform $\textbf{h}_{t}$ using a one layer Multi-Layer Perceptron (MLP) to obtain its hidden representation $\textbf{u}_{t}$. We assume Gaussian priors with $0$ mean and $0.1$ standard deviation on $\textbf{W}_w$ and $\textbf{b}_w$.
\begin{align} \label{eq:affine_word}
\textbf{u}_{t} = tanh(\textbf{W}_w \textbf{h}_{t} + \textbf{b}_w)
\end{align}
Next, to compute the importance of the word in the current context we calculate its relevance to a global context vector $\textbf{c}$ using a bilinear projection. 
\begin{align}
 f_{t} =  \textbf{c}^\top \textbf{W}_i \textbf{u}_{t} \label{eq:bil}
\end{align}
Here, $\textbf{W}_i \in {\rm I\!R}^{2h \times 2h}$, is a bilinear projection matrix which is randomly initialized and jointly learned with other parameters during training. $h$ is the dimension of the GRU hidden state and $\textbf{u}_t$ \& $\textbf{c}$ are both of dimension $2h \times  1$ since we're using a bi-GRU. The mean of the word embeddings provides a good initial approximation of the global context of the document. We initialize $\textbf{c} = \frac{1}{T}\sum_{t=1}^T \textbf{w}_t$ which is then updated during training. 
% In the experiments section we show that this initialization performs much better than random initialization.
We use a bilinear projection because they are more effective in learning pairwise interactions as shown in previous works ~\citep{chen2017reading}.  The attention weight for the word $\textbf{x}_{t}$ is then computed using a \textit{softmax} function where summation is taken over all the words in the document.
\begin{align} \label{eq:single_head}
   \alpha_{t} = \frac{exp(f_{t})}{\sum_{t'} exp(f_{t'})}
\end{align}
% We measure the importance of a word to the final representation by computing an alignment score of $\textbf{u}_{t}$ to a word level context vector $\textbf{u}_w$ using a bilinear model because bilinear models can be more effective in learning pariwise interactions especially for large feature-spaces: 
% \begin{align}
%  f_{t} =  \textbf{u}^T_w \textbf{W}_a \textbf{u}_{t} \label{eq:bil}
% \end{align}
% Here, $\textbf{W}_a$, a bilinear projection matrix, $\textbf{u}_w$ is randomly initialized and jointly learned with other parameters during training. Similar to ~\citep{han}, $\textbf{u}_w$ can be seen as a high dimensional representation of the fixed query `What is the informative word'. Having a bilinear projection matrix helps capture pairwise interactions between the context vector $u_w$ and the word representation $u_t$. $\textbf{u}_w \in {\rm I\!R}^l$, $\textbf{u}_{t} \in {\rm I\!R}^{2h}$ and $\textbf{W} \in {\rm I\!R}^{lx2h}$. 
% The attention mechanism normally used is sometimes referred to as multiplicative attention ~\citep{luong2015effective}. 
% \begin{align}
%     align(\textbf{h}_i, \textbf{s}_j) = \textbf{h}_i \textbf{W}_a \textbf{s}_j
% \end{align}
% We tried other variants of the attention mechanism such as additive attention as used in neural machine translation ~\citep{bahdanau+al-2014-nmt} which when simplified to compute unnormalized alignment scores for each hidden state $\textbf{h}_i$ is also know as self attention ~\citep{lin+al-2017-embed-arxiv}. For instance alignment scores for sentences can be obtained as $\alpha_i = \textbf{v}^T tanh( \textbf{W} \textbf{h}_i)$. Running extensive experiments using both variants of attention we find that multiplicative attention performs better.
% % First we get a variable length alignment vector $\textbf{a_s}$ whose size is equal to the length of the sentence, $T$.
% The attention weight for the word $\textbf{x}_{t}$ can be computed through a softmax function.
% \begin{align}
%   \alpha_{t} = \frac{exp(f_{t})}{\sum_{t'} exp(f_{t'})}
% \end{align}
% A sentence embedding is computed by taking a weighted average of the GRU hidden states.
% \begin{align}
% \textbf{s}_i = \sum_t \alpha_{it} \textbf{h}_{it}
% \end{align}

% Having a bilinear projection matrix gives us the flexibility to choose the dimension of $\textbf{u}_w$. In the results section we perform sensitivity analysis on the model by varying the dimension of $\textbf{u}_{w}$ to understand its impact on performance. We find that models with dimension of $\textbf{u}_w$ lower than $h$ seem to perform better. This may be because the model is trying to create a compact representation of the word features allowing it to store only the most important information.


\begin{table}[]
\caption{Important notations. Capital bold letters indicate matrices, small bold letters indicate vectors, small letters indicate scalars.}
\label{tab:note}
\small
\begin{center}
\begin{tabular}{|l|l|} \hline
\textbf{Notation} & \textbf{Meaning}  \\ \hline
 $N$ & Corpus size \\ 
 $T$ & \# of words tokens in a sample \\
 $m$ & \# of attention heads   \\
 $f_{t}$ & alignment score \\
 $\alpha_{t}$ & attention weight \\
 $\textbf{u}_{t}$ & word hidden representation \\
 $\textbf{c}$ & global context vector \\
 $h$ & GRU hidden state dimension \\
\hline
\end{tabular}
\end{center}
\vspace{-1em}
\end{table}

\begin{figure*}[ht!]
 \centering
 \small
  \includegraphics[width=\textwidth]{images/SDM_LAMA.pdf}
 \caption{Figure shows a schematic of the model architecture and its major components including the Sentence Encoder, proposed multi-head attention mechanism LAMA, Structured Sentence Embedding and finally the MLP classifier. The attention computation is demonstrated for a single word.}
 \label{fig:desc}
\vspace{-1em}
\end{figure*}

\subsection{Low-Rank Factorization based Multi-Head Attention}
\label{sec:lama}
In this section, we describe the novel low-rank factorization based multi-head attention mechanism (LAMA).
The attention distribution in Eq. ~\ref{eq:single_head} above usually focuses on a specific component of the document, like a special set of trigger words. So it is expected to reflect an aspect, or component of the semantics in a document. This type of attention is useful for smaller pieces of texts such as tweets or short reviews. For larger reviews there can be multiple aspects that describe that review.  For this we introduce a novel way of computing multiple heads of attention that capture different aspects.

Suppose $m$ heads of attention are to be computed, we need $m$ alignment scores between each word hidden representation $\textbf{u}_{t}$ and the context vector $\textbf{c}$. To obtain an $m$ dimensional output $\textbf{f}_{t}$, we need to learn $m$ weight matrices given by $\textbf{W} = [\textbf{W}_1, ...,\textbf{W}_m] \in \mathbf{R}^{m \times 2h \times 2h}$ as demonstrated in previous works. Although this strategy might be effective in capturing pairwise interactions for each aspect it also introduces a huge number of parameters that may lead to overfitting and also incur a high computational cost especially for a large $m$ or a large $h$. To address this, the rank of matrix $\textbf{W}$ can be reduced by using low-rank bilinear method to have less number of parameters ~\citep{kim2016hadamard,yu2017multi}. Consider one head; the bilinear projection matrix $\textbf{W}_i$ in Eq. \ref{eq:bil} can be factorized into two low rank matrices $\textbf{P}$ \& $\textbf{Q}$.

\begin{align}
 f_{t} = \textbf{c}^\top  \textbf{P}  \textbf{Q}^\top \textbf{u}_{t} = \sum_{d=1}^k \textbf{c}^\top p_d q_d^\top \textbf{u}_{t} 
 =   \mathbbm{1}^\top(\textbf{P}^\top \textbf{c} \circ \textbf{Q}^\top \textbf{u}_{t}) \label{eq:decompose}
\end{align}
where $\textbf{P} = [p_{1}, ..., p_{k} ]  \in {\rm I\!R}^{2h \times k}$ and $\textbf{Q} = [q_{1}, ..., q_{k}] \in {\rm I\!R}^{2h \times k}$ are two low-rank matrics,  $\circ$ is the Hadamard product or the element-wise multiplication of two vectors, $\mathbbm{1} \in {\rm I\!R}^k$ is an all-one vector and $k$ is the latent dimensionality of the factorized matrices.

To obtain $m$ scores, by Eq.\ref{eq:decompose}, the weights to be learned are two three-order tensors
$\mathds{P} = [\textbf{P}_{1}, ..., \textbf{P}_{m}] \in {\rm I\!R}^{2h \times k \times m}$ and $\mathds{Q} = [\textbf{Q}_{1}, ..., \textbf{Q}_{m}] \in {\rm I\!R}^{2h \times k \times m}$
accordingly. Without loss of generality 
$\mathds{P}$ and $\mathds{Q}$ can be reformulated as 2-D matrices $\Tilde{\mathds{P}} \in  {\rm I\!R}^{2h\times km}$ and $\Tilde{\mathds{Q}} \in {\rm I\!R}^{2h \times km}$ respectively with simple reshape operations. Setting $k=1$, which corresponds to rank-1 factorization. Eq.\ref{eq:decompose} can be written as: 
\begin{align} \label{eq:lama}
  \textbf{f}_{t} = \Tilde{\mathds{P}}^\top\textbf{c} \circ \Tilde{\mathds{Q}}^\top\textbf{u}_{t}
\end{align}
% Here $\textbf{U} \in  {\rm I\!R}^{lxm}$ and $\textbf{V} \in {\rm I\!R}^{2hxm}$ are two low rank matrices, $m$ is the number of aspects to extract and $\circ$ is the Hadamard product or elementwise multiplication.
This brings the two feature vectors $\textbf{u}_{t} \in \mathbf{R}^{2h}$, the word hidden representation and $\textbf{c} \in \mathbf{R}^{2h}$, the global context vector in a common subspace and are given by $\Tilde{\textbf{u}}_{t}$ and $\Tilde{\textbf{c}}$ respectively.
% Although this strategy might be be effective in capturing pair-wise  interactions  for  each  aspect  it  also  introduces  a  huge number of parameters that may lead to overfitting and also incur a high computational cost. Inspired by multi-modal low rank bilinear pooling approach proposed by Kim et. al ~\citep{kim2016hadamard} and the matrix factorization approaches proposed in ~\citep{li2017factorized, rendle2010factorization} the bilinear projection matrix $\textbf{W}_a$ can be factorized into two rank 1 matrices $\textbf{P}$ \& $\textbf{Q}$. Eq.\ref{eq:bil} can be written as: 
% \begin{align}
%   \textbf{f}_{t} =  \textbf{u}^T_w \textbf{W}_a \textbf{u}_{t} = \textbf{P}^T \textbf{u}_w \circ \textbf{Q}^T \textbf{u}_{t} = \Tilde{\textbf{u}}_w \circ \Tilde{\textbf{u}}_{t}
% \end{align}
% Here $\textbf{P} \in  {\rm I\!R}^{lxm}$ and $\textbf{Q} \in {\rm I\!R}^{2hxm}$ are two rank 1 matrices, $m$ is the number of aspects to extract and $\circ$ is the Hadamard product or elementwise multiplication.
% This brings the two feature vectors $\textbf{u}_{t} \in \mathbf{R}^{2h}$, the word hidden representation and $\textbf{u}_w \in \mathbf{R}^l$, the word level context vector in the common space
$\textbf{f}_{t} \in {\rm I\!R}^m$ can be viewed as a multi-head alignment vector for the word $\textbf{x}_{t}$ where each dimension of the vector can be viewed as the score of the word w.r.t. a different attention head. For computing attention for one head, this is equivalent to replacing the projection matrix \textbf{$\textbf{W}_i$} in Eq. ~\ref{eq:bil} by the outer product of vectors $\Tilde{\mathds{P}_i}$ and $\Tilde{\mathds{Q}_i}$;  rows of the matrices $\Tilde{\mathds{P}}$ and $\Tilde{\mathds{Q}}$ respectively and rewriting it as the Hadamard product. As a result each row of matrices $\Tilde{\mathds{P}_i}$ and $\Tilde{\mathds{Q}_i}$ represent the vectors for computing the score for a different head.

The multi-head attention vector $\bm{\alpha}_{t} \in {\rm I\!R}^m$ is obtained by computing a softmax function along the sentence length: 
\begin{align}
  \bm{\alpha}_{t} =  \frac{exp(\textbf{f}_{t})}{\sum_{t'} exp(\textbf{f}_{t'})}
\end{align}
Before computing softmax, similar to previous works ~\citep{kim2016hadamard,yu2017multi}, to further increase the model capacity we apply the \textit{tanh} nonlinearlity to $\textbf{f}_{t}$. Since element-wise multiplication is introduced the variance of the model might increase, so we apply an $l_2$ normalization layer across the $m$ dimension. Although $l_2$ is not strictly necessary since both $\textbf{c}$ and $\textbf{u}_t$ are in the same modality empirically we do see improvement after applying $l_2$. Each component $k$ of $\bm{\alpha}_{t}$ is the contribution of the word $\textbf{x}_t$ to the $k^{th}$ head.  

Next, we describe how this computation can be vectorized for each word in the document. Let $\textbf{H} = (\textbf{h}_{1}, \textbf{h}_{2},...\textbf{h}_{T})$ be a matrix of all word annotations in the sentence; $\textbf{H} \in {\rm I\!R}^{T \times 2h}$.
The attention matrix for the sentence can be computed as: 
\begin{align} 
\textbf{A} = softmax(l2(tanh(\tilde{\mathds{P}}^\top \textbf{C}_g\circ \tilde{\mathds{Q}}^\top  \textbf{H}^\top)))  \label{eq:attn}
\end{align}
where, $\textbf{C}_g \in  {\rm I\!R}^{2h \times T}$ is $\textbf{c}$ repeated $T$ times, once for each word, $l_2(\textbf{x}) = \frac{\textbf{x}}{||\textbf{x}||}$ and \textit{softmax} is applied row-wise. $\textbf{A} \in {\rm I\!R}^{m \times T}$ is the attention matrix between the sentence and the global context with each row representing attention for one aspect. 


% A sentence embedding for one aspect is computed by taking a weighted average of the GRU hidden states.
% \begin{align}
% \textbf{s}_{io} = \sum_t \alpha_{it} \textbf{h}_{it}
% \end{align}

Given $\textbf{A} = [\bm{\alpha}_{1}, \bm{\alpha}_{2},...\bm{\alpha}_{T}]$, the multi-head attention matrix for the sentence; $\textbf{A} \in {\rm I\!R}^{m \times T}$. The document representation for a head $j$ given by $\bm{\alpha}_{j} = \{\alpha_{j1}, \alpha_{j2},..\alpha_{jT}\}$ can be computed by taking a weighted sum of all word annotations.
\begin{align}
\textbf{s}_{j} = \sum_{k=1}^T \textbf{h}_{k}*\alpha_{jk}
\end{align}
Similarly, document representation can be computed for all heads and is given in a compact form by:
\begin{align}
    \textbf{S} = \textbf{A}\textbf{H} \label{eq:sent_emb}
\end{align}
Here $\textbf{S} \in {\rm I\!R}^{m\times2h}$ is a matrix sentence embedding and contains as many rows as the number of heads. Each row contains an attention distribution for a new head. It is flattened by concatenating all rows to obtain the document representation $\textbf{d}$. From the document representation, the class probabilities are obtained as follows.
\begin{align}
\hat{\textbf{y}} = softmax(\textbf{W}_c \textbf{d} + \textbf{b}_c)
\end{align}
Loss is computed using cross entropy. 
\begin{align}
L(\textbf{y}, \hat{\textbf{y}}) = -\sum_{c=1}^C y_c log(\hat{y_c})
\end{align}
where $C$ is the number of classes and $\hat{y_c}$ is the probability of the class $c$.
% The sentence embedding given by eq. \ref{eq:sent_emb} can suffer from redundancy issues if the attention mechanism always provides similar weights for all the $m$ aspects. To attend to a small set of trigger words in each aspect and to encourage diversity in different aspects we use penalization as described by Lin et al. ~\citep{lin2017structured} that is added to the loss: 
% \begin{align}
% P = \frac{\sum_i\left\lVert\textbf{A}_i\textbf{A}_i^T - \textbf{I}\right\rVert^2_F}{n} 
% \end{align}
% Where $\left\lVert \circ \right\rVert_{F}$ stands for the Frobenius norm of a matrix and the summation is taken over all sentences in the document. 

\subsection{Disagreement Regularization}
To reduce the variance of model introduced due to point-wise multiplication and to encourage diversity among multiple attention heads we introduce an auxiliary regularization term.
\begin{equation}
    J(\theta) = arg min_{\theta} \{ L(\textbf{y}, \hat{\textbf{y}}) - \lambda * D(\textbf{A} | \textbf{x}, \textbf{y}; \theta) \} \label{eq:loss}
\end{equation}
where \textbf{A} is the attention matrix, $\theta$ represents model parameters, $\lambda$ is a hyper-parameter and is empirically set to 0.2
in this paper. $L(\hat{\textbf{y}}, \textbf{y})$ is the cross-entropy loss and $D(\textbf{A} | \textbf{x}, \textbf{y}; \theta)$ is the auxiliary regularization term that represents the disagreement between different attentions. It guides the related attention components to capture different features from the corresponding projected subspaces.
We try two different regularizations i) regularization over attended positions ii) regularization over document embeddings. For the first type we adapt the penalization term in ~\citep{lin2017structured} to represent disagreement between attention distributions (Eq. \ref{eq:dpenal}).
% We try another type of disagreement over attended positions represented by the dot product between different attention distributions (Eq. \ref{eq:dpos}). Here, $\textbf{a}_i$ and $\textbf{a}_j$ are rows of the attention matrix $\textbf{A}$.
Next, we directly regularize the sentence embeddings resulting from different attention distributions represented using their cosine similarity (Eq. \ref{eq:demb}). The more similar the embeddings, lesser the disagreement.
\begin{subequations}
\begin{align}
     D_{penal} =  - \lVert \textbf{A}\textbf{A}^\top - \textbf{I} \rVert^2_F  \label{eq:dpenal} 
\end{align}
% \begin{align}
%     D_{pos} = -\frac{1}{m^2} \sum_{i=1}^m \sum_{i=1}^m \textbf{a}_i \cdot \textbf{a}_j \label{eq:dpos}
% \end{align}
\begin{align}
    D_{emb} = -\frac{1}{m^2} \sum_{i=1}^m \sum_{i=1}^m \frac{\textbf{s}_i \cdot \textbf{s}_j}{\lVert \textbf{s}_i \rVert \lVert \textbf{s}_j \rVert} \label{eq:demb}
\end{align}
\end{subequations}
The final training loss is given by Eq. \ref{eq:loss}
summed over all documents in a minibatch.
% \begin{align}
%     L = \sum_d l
% \end{align}
% \begin{align}
%     L = \sum_d l + \lambda P
% \end{align}
We use the minibatch stochastic gradient descent algorithm ~\citep{kiefer1952stochastic} with momentum and weight decay for optimizing the loss function and the backpropogation algorithm is used to compute the gradients. 

Fig. \ref{fig:desc} shows a single document and its flow through various model components. The middle block illustrates the proposed attention mechanism for one word $\textbf{w}_t$ of the document. It is first transformed through Eq. ~\ref{eq:affine_word} to $\textbf{u}_t$. In parallel, a context vector $\textbf{c}$ is initialized. Eq. ~\ref{eq:lama} is then used to compute the multi-head attention for this word. Vectorized attention computation can be performed for all words using Eq. ~\ref{eq:attn}  to obtain the attention matrix $\textbf{A}$ which is then multiplied by the hidden state matrix $\textbf{H}$ to obtain an embedding for the document which is then passed to the MLP classifier.

% \begin{algorithm2e}
% \SetAlgoLined
% \scriptsize
% \KwResult{One update to the model parameters}
% \SetKwInOut{Input}{Input} \SetKwInOut{Output}{Output}
% \Input{Tokenized input batch}
% % \Output{Attention matrix}
% %  \While{Loop throug}{
% %  $j\leftarrow0$\;
%  \while{loop through each batch of the train dataset}{
%  Get the word embedding for each token via a look up into the embedding matrix ;\
%  Compute the context vector $C_g$ if using LAMA + Ctx else initialize $C_g$ \;
%  Get the hidden states matrix $H_i$ of the sentence via a bi-GRU \;
%  Compute the attention matrix $A$ using Eq. ~\ref{eq:attn} \;
%  Get the sentence embedding using Eq. ~\ref{eq:sent_emb} and flatten the embedding \;
%  Pass the flattened embedding through a fully-connected layer, followed by a softmax \; 
%  Compute the cross entropy loss obtained from the resulting logits \;
%  Compute gradient updates to the model parameters using the backpropogation algorithm
%  }
%   \caption{Algorithm describing computation in one epoch for }
%   \label{alg:causalInterconnection}
% \end{algorithm2e}
% \subsubsection{Phrase-Level Context}
% A noteworthy effect of bringing the global context vector and word representations in a low-dimensional common subspace is that the words appearing frequently together tend to get similar attention weights. Words that appear together have similar relevance to the global context and therefore get close attention weights. Note also, that the global context vector is initialized using word2vec ~\citep{mikolov2013distributed} which is trained to predict the surrounding context of a word. So initializing $\textbf{c}$ using the mean of word embeddings strengthens this effect.

\subsection{Hyperparameters}
We use a word embedding size of 100. The embedding matrix $\textbf{W}_e$ is pretrained on the corpus using word2vec ~\citep{mikolov2013distributed}. All words appearing less than 5 times are discarded. The GRU hidden state is set to $h=50$, MLP hidden state to $512$ and we apply a dropout of $0.4$ to the hidden layer. Batch size is set to $32$ for training and an initial learning rate of $0.05$ is used. For early stopping we use $patience=5$. Momentum is set to 0.9 and weight decay to 0.0001. 
% We have open sourced our code and is available here ~\footnote{https://github.com/sumehta/LAMA}.
We will open source the code on acceptance. 
% and is available here  \footnote{https://github.com/xkcd456/LAMA}.

\subsection{Computational Complexity}
Other variables such as document encoder and dimension of the hidden state held constant, the computational complexity of the model depends on the attention layer. It can be seen that the computational complexity of LAMA is linear in input and linear in the number of attention heads. Where as, the attention mechanism in the encoder of a Transformer model ~\citep{vaswani2017attention} is quadratic in the length of the input (Table ~\ref{tab:complexity}). For cases where $n*m \ll n^2$, which is a common scenario, attention mechanism LAMA is computationally more efficient than self-attention in encoder of the Transformer model for sequence classification tasks.

\begin{table}[]
\centering
\caption{\small{Per-layer complexity for different layer types. $n$ is the document length, $m$ is the number of attention heads and $d$ is the representation dimension.}}
\label{tab:complexity}
\begin{tabular}{@{}ll@{}}
\toprule
Layer Type          & Complexity per Layer \\ \midrule
Self Attention (LAMA)               &    $O(n*m*h)$                  \\
Self-Attention (TE) &   $O(n^2*d)$                \\
% Self-Attention (SAN)      &  $O(n*m*d)$                   \\
\bottomrule
\end{tabular}
\end{table}
% \subsubsection{Parameter Size}
% For h=100, d=100, the bilinear attention or multiplicative attention proposed in eq. \ref{eq:bil} $W_i$ would have a dimension of $100x100$. Whereas, in FBMA, for $m=10$, $\textbf{P}$ would have a dimension of $100x10$ and $\textbf{Q}$ would have a dimension of $100x10$.
% \begin{figure}[t!]
%  \centering
%   \includegraphics[width=0.47\textwidth]{images/model.pdf}
%  \caption{\small{An illustration of the model architecture. The FBMA component is used at the word level to get the matrix sentence embedding.}}
%  \label{fig:model}
%  \vspace*{-0.2in}
%  \end{figure}

% \begin{table*}
%   \caption{Model Hyperparameters}
%   \label{tab:hyp}
%   \begin{center}
%  \begin{tabular}{|c c c|} 
%  \hline
%  N & batch size & 64 \\  
%  max_words & 
%  max_sents &
%  hidden_dim &
 
%  \hline\hline
%  &
%  &
%  \\ 
%  \hline
%  &
%  &
%  \\ 
%  \hline
%   &
%   &
%  \\ 
%   \hline
% \end{tabular}
% \end{center}
% \end{table*}
% \subsection{Cross-Lingual Embeddings}

% \section{Key Sentence Extraction}









% \section{Title embedding}


% \section{Multiple Instance Learning} 
% LSTM/CNN Model and its results



% \section{Multilingual Transfer Learning}
% Multi Task Models:
% Problem characteristic - The inputs for both tasks (protest type and population type are the same, but intuitively there should be some shared attention layers that learn to attend towards protest specific keywords and some task specific attention layers that learn to attend to task specific keywords. 

% The text Encoder will be shared.

% Multi-head attention - a few heads with be shared, a few heads will be separate. 

% shared heads will be concatenated with the task-specific heads finally to compute task specific loss which is will be backpropogated.

% Naive Bayes results for positive only:
% Naive Bayes PRT Only positive
% prec- 0.20130070728673655
% rec - 0.4100286326370865
% f1 - 0.1815858851946561
% acc - 0.5761245674740484



% \section{Detecting Event Type and Population Type}
% After detecting the key sentences containing the event and the key words related to the event, it is useful to detect the type of the protest event (event types are listed in table \ref{tab:tp}) and the sect of the population participating in the event (population types are listed in \ref{tab:pop}. For a small subset of the original AutoGSR dataset (the GSR subset) we have labels indicating the population and the event type. This can also be formulated as a standard classification problem. We model this using the various comparative methods and the HAN model with number of classes now set to five and eleven respectively corresponding to both the problems.



% \begin{itemize}
%     \item  MIL approach with bi-LSTM sentence encoder and penalizing attention weights (gives good results with good attention words) (1)
%     \item Transfer weights from all but classifier layers for the task of population type and protest type (2)
% \end{itemize}

% Things to try
% \begin{itemize}
%     \item Use title information to improve performance of item 1 above.
%     \item Improve transfer learning performance for popt and prt (popt and prt words should be attended to)
%     \item Use supervised attention to improve performance of popt and prt above 
%     \item Use transformer-encoder for improved performance (this item is in a separate group from above three)
% \end{itemize}



% \section{Multiple Instance Learning Loss}
% Below we describe how we extend our multiple instance learning architecture for multiple classes.

% For each sentence in an article we get the probability for each of the 5 protest classes, we aggregate the probability of the topk sentences for each class. i.e. we aggregate the probabilities of the most confident K sentences for each protest class. Finally we get the softmax loss as:

% \begin{align}
% \text{loss}(x, class) = -\log\left(\frac{\exp(x[class])}{\sum_j \exp(x[j])}\right)
%                       = -x[class] + \log\left(\sum_j \exp(x[j])\right) 
% \end{align}


% \section{Proposed Model}
% If we train separate for models for each task, the top ranked event sentences in each case are different. We train our best performing model on all three tasks, table 3 shows the statistics of how many times the top ranked sentence is same for all three tasks, and for tasks pairwise.

% % During training phase we are given a set of news articles containing event of interest, location and time of the event. At test time the task is to assign event roles to entities if the article mentions the event. Given an article, at test time each entity in the article is assigned an event role Location, Time, or None in the test article.

% % Detecting population type: The Population Type role of an event does not consist of entities but a set of key words and each event could have one of eleven population types. Each keyword belonging to each of the eleven population types are considered as entities and those entities are assigned to one of 11 population type roles in table 2. 

% Protest type and Population type of an event are tied to each other in that the same sentences will contain information  both. To model this we propose a Multi-Task framework in which sentence attention weights are shared for both tasks. Finally the shared layers between both tasks consist of sentence encoder, and sentence attention weights. Each task gets its own word attention layer because words relating to protest type and population type are different. 

% Finally we add an additional task of predicting event span as an auxiliary task. Sentences containing protest type and population type information are highly likely to be sentences containing the event mention.

% Given an article $x = {x_1, x_2,...,x_n}$ consisting of $n$ sentences and associated labels $l_r$, $l_p$, $l_o$ where $l_p \in {0, 1}$, $l_r \in {0,...,6}$ and $l_o \in {0,...,12}$, $l_p$ indicating whether a given article talks about a protest event or not, $l_r$ indicating one of five protest types or a non-protest article and $l_o$ indicating one of 11 population types or a non-protest article. Our aim is to jointly predict whether an article is a protest article or not, predict its protest type and population type.



% We show that our approach works on protest datasets in two languages.
% Terminology:
% \begin{itemize}
%     \item Entity: An Entity is dened as an object or set of objects in the world. E.g., Micorsoft is a company entity and Anonymous is a organization entity.
%     \item Entity Mention: Entity mention is a reference to the entity in the text. E.g., each appearance of Micorsoft in one article is a mention for Microsoft entity.
%     \item Event Extent:: An Event extent is a sentence within which a specic event is described.
%     \item Event Argument: Event argument is an entity mention, which will be a participant or an attribution in the event.
% \end{itemize}


% Model:
% HAN capturing document  - event extent 
% An entity bag - 



% Contributions:
% - Attention-based model for extracting key sentences
% - Using key sentences to predict population type and protest type
% - Transfer learning from for improving performance
% - Adding title embeddings
% - Using supervised attention
% - Using multi-lingual transfer

% \subsection{Model size}
% We compare the computational efficiency of our embedding to the structured embedding proposed by Lin et. al. ~\citep{lin2017structured}. Specifically we compare the number of parameters needed to compute a multi-aspect attention vector for one word. Let $D=\{w_1, w_2,...,w_T\}$ be a document consisting of T words. Consider a word $w_i \in D$. Let $\textbf{H}$ be the matrix of bi-GRU hidden states. $\textbf{H} \in {\rm I\!R}^{Tx2h}$ where $h$ is the dimension of the GRU hidden state. According to Lin et. al. 
% \begin{align}
%   \textbf{A} = softmax(\textbf{W}_{s_2}tanh(\textbf{W}_{s_1}\textbf{H}^T))
% \end{align}
% where, $\textbf{W}_{s_1}$  is a weight matrix with a shape of $d_a$-by-2h and $\textbf{W}_{s_2}$ is  r-by-$2h$.
% So the total number of parameters required to compute attention for 1 word is,
% \begin{align}
% d_a x 2h + r x 2h
% \end{align}
% where $r$ is the number of aspects.

% For the proposed model, the only parameters required to compute attention for one word are matrices \textbf{P} and \textbf{Q} where \textbf{P} is l-by-m and \textbf{Q} is 2h-by-m.  So the total number of parameters required are,
% \begin{align}
% lxr + 2hxr,
% \end{align}
% where r is the number of aspects.
% Now comparing the above equations, we can ignore the second term. In the first term, assuming $l$ the dimension of the context vector and $d_a$ to be equal, the reduction factor is $\frac{d_a}{r}$. If we consider 5 aspects and 350 as the size of $d_a$ as used in their paper our model uses 70 times fewer parameters.

% Most of the gains of our model are coming from factorization of matrix $\textbf{W}$ into low rank matrices $\textbf{P}$ \& $\textbf{Q}$. If not for this, our model reduces to a single aspect self attentive model where $\textbf{W}_{s1} = \textbf{W} \oplus \textbf{u}_w$ ; $\oplus$ represents the concatenation operator. 

==> CIKM 2020/sections/results.tex <==
\section{Evaluation} \label{sec:experiments}

\subsection{Datasets}
We evaluate the performance of the proposed model on tasks of predicting business ratings from Yelp, sentiment prediction from movie reviews and classifying news articles into topics.  Table ~\ref{tab:dataset} gives an overview of the datasets and their statistics. 

\begin{table}[]
\centering
\caption{Dataset statistics. \# words indicates the average number of tokens per document in the corresponding datasets.}
  \label{tab:dataset}
\begin{tabular}{lllll}
Dataset & \# Classes & \# Train & \# Test & \# words \\ \hline
YELP & 5 & 499,976 &  4,000 & 118  \\
YELP-L & 5 & 175,844 & 1,378 & 226 \\
YELP-P & 2 & 560,000 & 38,000 & 137 \\ 
% Amazon & 5 & 499,987 & 50,000 & 79\\
IMDB & 2 & 25,000  & 25,000 & 221 \\
Reuters & 8 & 4,484 & 2,189 & 102 \\
% MANSA & 74,100  & 15,880 & 1575\\
News & 4 & 151,328  & 32,428  & 352  \\ \hline
\end{tabular}
\end{table}

% \subsection{Review Ratings}
% For the sentiment analysis task we pick two datasets - the YELP Ratings dataset and the IMDB Movie Sentiment Dataset.

\subsubsection{Yelp}
The Yelp dataset ~\footnote{https://www.yelp.com/dataset challenge}  consists of 2.7M Yelp reviews and user ratings from 1 to 5. Given a review the goal is to predict the rating assigned by the user to the corresponding business store. We treat the task as 5-way text classification where each class indicates the user rating. We randomly sampled 500K review-star pairs as training set and 4,000 for test set. Reviews were tokenized using the Spacy tokenizer ~\footnote{https://spacy.io/}. 100-dimensional word embeddings were trained from scratch on the train dataset using the gensim ~\footnote{https://radimrehurek.com/gensim/} software package. 
% dev set contains 4000 reviews
\subsubsection{Yelp-Long}
Multi-head attention capturing multiple aspects is more useful for classifying ratings that are more subjective i.e. longer reviews where people express their experiences in detail. We create a subset of the YELP dataset containing all longer reviews i.e. reviews containing longer than 118 tokens which we found to be the mean length of the reviews in the dataset. The training set consists of 175,844  reviews, and the test set consists of 1,378 reviews. The goal is to predict the ratings from the above subset of the Yelp dataset. We refer to this dataset as Yelp-L (Yelp-Long) in the rest of the paper since it consists of all longer reviews. We hypothesize that having multi-head attention would benefit in this setting where more intricate foraging of information from different parts of the text is required to make a prediction.
The model hyperparameters and training settings remain the same as the above.
% dev set consists of 1,416 reviews

\subsubsection{Yelp-Polarity}
The Yelp reviews polarity dataset ~\citep{zhang2015character} is constructed by considering stars 1 and 2 negative, and 3 and 4 positive from the Yelp dataset. For each polarity 280,000 training samples and 19,000 testing samples are taken randomly. In total there are 560,000 training samples and 38,000 testing samples. This datset is referred as Yelp-P in the paper.

% \subsubsection{Amazon Ratings}
% The Amazon reviews dataset ~\citep{zhang2015character} consists of plain text product reviews, their ratings from 1 to 5 stars and their title. For the purposes of this paper we uniformly sample 100,000 samples per rating from train split to construct our train dataset of ~500K reviews and 10,000 from test split to construct our test dataset of 50,000 reviews.

\subsubsection{Movie Reviews}
The large Movie Review dataset ~\citep{maas-EtAl:2011:ACL-HLT2011} contains movie reviews along with their associated binary
sentiment polarity labels. It contains 50,000 highly polar reviews ($score \leq 4$ out of 10 for negative reviews and $score >= 7$ out of 10 for positive reviews) split evenly into 25K train
and 25K test sets. The overall distribution of labels is balanced (25K pos and 25K neg).
In the entire collection, no more than 30 reviews are allowed for any given movie because reviews for the same movie tend to have correlated ratings. Further, the train and test sets contain a disjoint set of movies, so no significant performance is obtained by memorizing movie-unique terms and their associated with observed labels. 
%From the training set we randomly set aside 1000 reviews for validation. 
We refer to this dataset as IMDB in the rest of the paper.

% \subsubsection{SST2}
% \subsection{Event Detection}
% Event detection refers to identification of documents containing a specific event. It can be categorized as a hierarchical task where the coarser level task is event detection -- identification of documents containing a specific event and the fine-grained task of event encoding -- identifying key phrases, key sentences describing event related information like type of the event, type of people involved in the event and extracting relationships between those. Hierarchical attention networks (HAN) ~\citep{han} seem like a natural choice for this problem given their ability to differentially attend to more or less important features when constructing the document representation. Given a news article we aim to predict if it contains an event or not. This can be considered as a binary text classification task. For evaluation, in the HAN model, we replace the word-level attention with the proposed multi-aspect attention mechanism. The matrix sentence embedding obtained is flattened and input to the GRU sentence encoder (please refer to their paper for model details). For another baseline we replace the word-level attention with the self attentive attention mechanism.~\citep{lin2017structured}. We refer to this model as HSA. Finally we use the original HAN model as another baseline.

% The dataset we use for this task is the Military Action and Non-State Actor (MANSA) GSR dataset which is in English and Arabic. This contains event encodings from gulf countries namely, Bahrain, Egpyt, Iraq, Jordan, Lebanon, Qatar, Saudi Arabia and Syria. The event types include `Military Actions' (MA) which are actions by military, police, or security organization and `Non-State Actor'(NSA) which are actions initiated by non-governmental groups or individuals to further political, social, religious or ideological objectives. These events are encoded from news articles collected from the web and print media. Event collection techniques include Google Advanced Search (limited to the newspaper website), Nexis queries, and IHS Janes. Google Advanced Search is used to collect events in online media. Nexis and IHS Janes are used to collect events in print media. About 34\% articles describe an event and rest are non-event articles. We refer to this dataset as MANSA dataset in the paper. MA \& NSA events are further divided into subtypes. In this work we combine NSA \& MA events together for detection.

% \subsection{Author Profiling}
% This Author Profiling dataset ~\footnote{https://pan.webis.de/clef18/pan18-web/author-profiling.html} consists of tweets from 436 Twitter users in English, Spanish, and Dutch and belonging to five different age groups 18-24, 25-34, 35-49, 50-64, 65+. The task is to predict the age group given the tweet. We consider this as a multiclass classification problem with five classes. We randomly select 150,000 tweets for training, 4,000 for test and 4,000 for validation. We refer to this as the Age dataset in the rest of the paper.


% \subsection{News Classification}
% For this task we selected two datasets. 

\subsubsection{News Aggregator} This dataset  ~\citep{Dua:2017} contains headlines, URLs, and categories for news stories collected by a web aggregator between March 10th, 2014 and August 10th, 2014. News categories included in this dataset include business; science and technology; entertainment; and health. Different news articles that refer to the same news item are also categorized together. Given a news article the task is to classify it into one of the four categories. Training dataset consits of 151,328 articles and test dataset consits of 32, 428. The average token length is 352.

\subsubsection{Reuters}
This dataset \footnote{https://www.cs.umb.edu/smimarog/textmining/datasets/} is taken from Reuters-21578 Text Categorization Collection. This is a collection of documents that appeared on Reuters newswire in 1987. The documents were assembled and indexed with categories. We evaluate on the Reuters8 dataset consisting of news articles about 8 topics including acq, crude, earn, grain, interest, money-fx, ship,trade.


\subsection{Comparative Methods}
To benchmark the proposed model against existing methods we use a variety of model architectures as our comparative baselines.
We use BERT ~\citep{devlin2018bert} as one of the baselines. In our experiments, we used the pretrained bert-base uncased model which has 12-layers, 768-hidden state size, 12-heads, 110M parameters and is trained on lower-cased English text. We finetuned it on our datasets for 2 epochs using the ADAM optimizer ~\citep{kingma2014adam} with a learning rate of $5e-6$. 

It has been shown that average of word embeddings can make for a very strong baseline ~\citep{shen2018baseline}. We use this as another baseline and refer to it as AVG in the paper.

We use a variety of models with and without attention as other baselines. Strong representative baselines for different model architectures are chosen; such as CNN with \textit{max-over-time} pooling ~\citep{kim2014convolutional}, bidirectional GRU ~\citep{Chung2014EmpiricalEO} model with maxpooling referred as BiGRU. We experimented with $n=1$ and $n=2$ GRU layers and found that $n=1$ converged faster and led to a better performance. For the CNN baseline we used 3 kernels of sizes 3, 4 and 5 with 100 filters each.
% We choose a variety of models with and without attention for evaluation as our baselines. The first baseline is a simple average of word embeddings  . We refer to this as AVG in the rest of paper. 
% We use a bi-GRU ~\citep{Chung2014EmpiricalEO} model with maxpooling referred as BiGRU as a baseline.
% first we encode the given text with a bi-GRU and then take max over all hidden states of the GRU giving us a fixed sized sentence embedding.
% We use a 2-layer MLP classifier for prediction.
% We use a convolutional neural network with \textit{max-over-time} pooling ~\citep{kim2014convolutional} as another baseline. We refer to this  as CNN in the paper. 
% We use three kernels of size 3,4 \& 5 with 100 filters each.
% Among attention based methods, we fist use a single-head attention mechanism based on the dot-product
% used by Yang et al. ~\citep{han} as a part of their hierarchical attention networks (HAN) as one of the baselines. For a fair comparison we use a flat model and use attention at the word level to get the document embedding. We refer to this as HAN in the paper. 

Among supervised attention-based multi-head models we use the Self Attention Network proposed by Lin et al. ~\citep{lin2017structured}. We refer to this baseline as SAN. For each task, we empirically find the number of heads that give the best performance.  We use a 1-layer Encoder of the Transformer model (TE) ~\citep{vaswani2017attention} with 8 attention heads as another baseline.  We use $d_{model}=512$ such that $d_{model}/\text{heads} = 64$. 

We use two variations of the proposed model to compare the performance with the above baselines. For the first variation we initialize $\textbf{c}$ with mean of  word embeddings in the sentence to provide the global context of the sentence. We call this baseline \textsf{LAMA+ctx}. In another variation, we randomly initialize $\textbf{c}$ and jointly learn it with other model parameters (\textsf{LAMA}). Our model with embedding regularization is referred as \textsf{LAMA+ctx}+$d_{e}$ and our model with regularization over positions is referred as \textsf{LAMA+ctx}+$d_{p}$. For the models \textsf{LAMA} and \textsf{LAMA+ctx} we empirically identify the optimal number of attention heads to get the best performance. 
% For all models we use the default parameters i.e., $r=30$ and MLP hidden size is 3000. 
% For the MANSA dataset, which is a hierarchical classification task, we modify the HAN model by replacing the word-level attention with the proposed attention mechanism. For another baseline we replace the word-level attention in HAN with the self attentive attention mechanism ~\citep{lin2017structured}. We refer to this model as HSA. Finally we use the original HAN model as another baseline.
% We test these baselines against our model with the context vector initialized with the mean of the word embeddings (Our Model+ctx) in the sentence as well as random initialization from a uniform distribution (Our Model).

% Another baseline we use is the BERT model to compare against Transformer-based multi-head attention ~\citep{devlin2018bert}. However it should be noted that BERT is pretrained on a large external corpora and hence is an unsupervised method as opposed to our model which is completely trained from srcatch. For the BERT-baseline we use a pretrained BERT implementation ~\footnote{https://gluon-nlp.mxnet.io} and finetune it with a task-specific classifier. We finetune this classfier for 10 epochs using the ADAM optimizer with a learning rate of 5e-6. This baseline is referred to as BERT. For a fair comparison we do not use any creative pretraining techniques for BERT and use the original pretraining method introduced in the paper. ~\citep{sun2019fine,liu2019roberta}.  

% \begin{table}[!ht]
% \caption{\small{Various baselines and their key characteristics.}}
% \label{tab:methods}
% \small
% \centering
% \begin{tabular}{@{}lllll@{}}
% \toprule
% \begin{tabular}[c]{@{}l@{}}Features/\\ Baselines\end{tabular} & \begin{tabular}[c]{@{}l@{}}Bidirectional\\ context\end{tabular} & \begin{tabular}[c]{@{}l@{}}Bilinear \\ Attn\end{tabular} & \begin{tabular}[c]{@{}l@{}}Multi-Aspect\\ Attn\end{tabular} & No-Pretrainig \\ \midrule
% AVG                                                           & $\times$                                                        & $\times$                                                 &  $\times$                                                    &    $\checkmark $          \\
% CNN                                                           & $\times$                                                        & $\times$                                                 & $\times$                                                    &     \checkmark          \\
% BiGRU                                                         & \checkmark
% & $\times$                                                 & $\times$                                                    &  \checkmark             \\
% HAN-Flat                                                      & \checkmark                                                                & $\times$                                                 & $\times$                                                    &    \checkmark           \\
% SA                                                            &   \checkmark & $\times$                                                 &  \checkmark & \checkmark               \\
% BERT                                                          &  \checkmark & $\times$                                                 &  \checkmark & $\times$      \\
% \begin{tabular}[c]{@{}l@{}}LBP-Attn \\ (Ours)\end{tabular}    & \checkmark   &   \checkmark                                                       &   \checkmark & \checkmark \\ \bottomrule
% \end{tabular}

% \end{table}

% \begin{table}
% \caption{\small{Various baselines and their key characteristics.}}
% \label{tab:methods}
% \scriptsize
% \begin{tabular}{|l|ccccc|} \hline
% \textbf{Feature} & \textbf{hierarchical} &  \textbf{key}  & \textbf{key}  & \textbf{bilinear} & \textbf{multi-aspect} \\ 
% Method  &   &  \textbf{words} & \textbf{sents} & \textbf{attention} & \textbf{attention} \\ \hline

% HAN-Flat         & \checkmark & $\times$ &  \checkmark  &  $\times$   &   $\times$  \\
% SA       & \checkmark  & \checkmark  &  \checkmark & $\times$  &  $\times$   \\
% BiGRU          & \checkmark &  \checkmark  &  \checkmark  &  $\times$ &   $\times$               \\
% CNN          & \checkmark  & \checkmark  &  \checkmark & \checkmark  & $\times$\\
% AVG & \checkmark  & \checkmark  &  \checkmark & $\times$  & \checkmark \\
% LBP-Attn& \checkmark  & \checkmark &  \checkmark & \checkmark & \checkmark \\ \hline      
% \end{tabular}
% \end{table}

\section{Results} \label{sec:results}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}llllll@{}}
% \toprule
% Datasets  & Methods         & Precision & Recall & F1(Macro) & F1(Micro) \\ \midrule
%           & Han-Flat        &           &        &           &           \\
%           & SA              &           &        &           &           \\
%           & bi-GRU          &           &        &           &           \\
% News      & CNN             &           &        &           &           \\
%           & AVG             &           &        &           &           \\
%           & Our Model       &           &        &           &           \\
%           & Our Model + ctx &           &        &           &           \\ \midrule
%           & Han-Flat        &           &        &           &           \\
%           & SA              &           &        &           &           \\
%           & bi-GRU          &           &        &           &           \\
% Reuters   & CNN             &           &        &           &           \\
%           & AVG             &           &        &           &           \\
%           & Our Model       &           &        &           &           \\
%           & Our Model + ctx &           &        &           &           \\ \midrule
%           & Han-Flat        &           &        &           &           \\
%           & SA              &           &        &           &           \\
%           & bi-GRU          &           &        &           &           \\
% Yelp      & CNN             &           &        &           &           \\
%           & AVG             &           &        &           &           \\
%           & Our Model       &           &        &           &           \\
%           & Our Model + ctx &           &        &           &           \\ \midrule
%           & Han-Flat        &           &        &           &           \\
%           & SA              &           &        &           &           \\
%           & bi-GRU          &           &        &           &           \\
% Yelp-L & CNN             &           &        &           &           \\
%           & AVG             &           &        &           &           \\
%           & Our Model       &           &        &           &           \\
%           & Our Model + ctx &           &        &           &           \\ \midrule
%           & Han-Flat        &           &        &           &           \\
%           & SA              &           &        &           &           \\
%           & bi-GRU          &           &        &           &           \\
% IMDB      & CNN             &           &        &           &           \\
%           & AVG             &           &        &           &           \\
%           & Our Model       &           &        &           &           \\
%           & Our Model + ctx &           &        &           &           \\ \midrule
%           & Han-Flat        &           &        &           &           \\
%           & SA              &           &        &           &           \\
%           & bi-GRU          &           &        &           &           \\
% MANSA     & CNN             &           &        &           &           \\
%           & AVG             &           &        &           &           \\
%           & Our Model       &           &        &           &           \\
%           & Our Model + ctx &           &        &           &           \\ \bottomrule
% \end{tabular}
% \end{table}


\begin{table*}[!t]
\caption{\small{Table reports the accuracy of the proposed models (\textsf{LAMA}, \textsf{LAMA+ctx}) against various baselines on sentiment analysis and news classification tasks. $+D_p$ refers to \textsf{LAMA + Ctx} with position-wise regularization whereas $+D_e$ refers to \textsf{LAMA + Ctx} with regularization over embeddings.  }}
\label{tab:performance}

\centering
\begin{tabular}{@{}l|lllllll@{}}
\toprule
Methods      & News  & Reuters & Yelp  & IMDB  & Yelp-L & Yelp-P  \\ 

% \midrule
% Supervised & & & & -& \\ 
\midrule 
% HAN              & 0.915 & 0.971   & 0.71  & 0.895 &  0.655     \\
SAN (Lin et al. ~\citep{lin2017structured})                 & 0.876 & 0.942   & 0.68  & 0.831 &  0.638 & 0.945 \\
BiGRU                 & 0.905 & 0.867   & 0.663 & 0.876 &  0.608 & 0.943    \\
CNN (Kim et al. ~\citep{kim2014convolutional})                 & 0.914 & 0.96    & 0.693 & 0.874 & \textbf{0.672}  & 0.953  \\
TE (Vaswani et al. ~\citep{vaswani2017attention})                 & 0.899 &  0.901  &  0.655& 0.817  &  0.569  & 0.925 \\
BERT (Devlin et al. ~\citep{devlin2018bert})                &    0.92   &   0.97     &  0.715     &    0.894   &    \textbf{0.672}  & \textbf{0.97}  \\
AVG (Arora et al. ~\citep{arora2017asimple})                & 0.91  & 0.795   & 0.653 & 0.874 &   0.652 & 0.928  \\
\textsf{LAMA}  & 0.922 & 0.965   & 0.697 & 0.895 &   0.653 & 0.947\\
\textsf{LAMA + Ctx}  & \textbf{0.923} & \textbf{0.973}   & \textbf{0.716} & \textbf{0.90}   & 0.665 & 0.952   \\

    + $D_{p}$&  0.903   & 0.948 & 0.711 & 0.874 & 0.656 & 0.948 \\
% \textsf{LAMA + Ctx} + $D_{pos} $ & 0.903 & 0.947 &  0.704 & 0.839 & 0.665 & 0.949 \\
+ $D_{e} $ & 0.91 & 0.831  & 0.677 &  0.805 & 0.619 & 0.893 &   \\
% \midrule
% Unsupervised & &  & & & \\ 
% \midrule 
 \bottomrule
\end{tabular}
%\vspace*{-0.2in}
\normalsize
\end{table*}

Table ~\ref{tab:performance} reports the accuracy of the best model on the test set after performing 3-fold cross-validation. 
The proposed model with global context initialization \textsf{LAMA+ctx} outperforms the SAN model ~\citep{lin2017structured} on all tasks from 3.3\% (Reuters) to 8.2\% (IMDB). This is due to the fact that during attention computation the proposed model architecture has the provision to access the global context of the sentence whereas for SAN no such provision is available.
% 5.4\% (News), 3.3\% (Reuters) 5.3\% (Yelp) and 4.2\% (Yelp-L) . This improvement occurs with at least 70 times fewer parameters as demonstrated in section 3.3.
% This is because SA forces attention on individual words due to the penalization term whereas our model attends to phrases. 

% Word relevance can vary depending on the context. 

% See Fig. for an example from the Reuters dataset.

% \textcolor{Huzefa}{add SA vs Our model}

Extrapolating the attention over larger chunks of text we get uniform attention over all words, which is equivalent to no attention or equal preference for all words. This is what a simple BiGRU effects to (in a contextual setting and average of word embeddings in a non-contextual setting). We note that \textsf{LAMA+ctx} outperforms BiGRU by 2.0\% (News), 12.2\% (Reuters) 7.9\% (Yelp) and 9.4 \% (Yelp-L) and 2.7 \% (IMDB). 

Our models outperform the Transformer Encoder (TE) on all tasks. It should be noted that this performance improvement also comes with fewer parameters than TE (Table ~\ref{tab:param_vs_m}). When compared to large fine-tuned pre-trained language models such as BERT we find that LAMA outperforms BERT on News, Reuters, Yelp and IMDB datasets. On YELP-L and YELP-P datasets BERT outperforms LAMA. However, it should be noted that besides being trained on large-scale text corpora and having a large memory footprint compared to LAMA, BERT models also take a longer time for pretraining. For instance, for Yelp-P it took 12.5 hours to train the model just for 1 epoch as compared to 20 mins for LAMA and for Yelp it took 8.5 hours as opposed to 25 mins for LAMA on one Nvidia Tesla P100 GPU.
% News - 2:35:42, Reuters - 04:27, 
% Yelp - 8.5 hrs
 

% This improvement is lower as compared to the SA model which implies that these tasks prefer attention to larger chunks of text rather than smaller chunks but also tells us that attention is better than no-attention. Our model achieves this fine balance with regards to the attention structure.

For the non-contextual baseline of average of word embeddings there's an improvement of  1.4\% (News), 22.4\% (Reuters) 9.8\% (Yelp), 11.4\% (Yelp-L) and 3.0\% (IMDB)
which shows that contextual information captured by BiGRU or CNN models are indeed important for the tasks.

Compared to CNN models an improvement of 1\% (News), 1.4\% (Reuters) and 3.3\% (Yelp), and 3.0 \% (IMDB) can be observed.
% 4.3\% (Yelp-L), run CNN baseline
On the Yelp-L dataset our model and CNN perform similarly. However, the proposed model is more interpretable and gives an option for inspecting the attended keywords.

Finally, our results suggest that using disagreement regularization on LAMA worsens the performance in general.

From the above results it can be noted that LAMA is a competitive, interpretable and lean supervised model for text classification tasks. 
% This could be explained due to the fact that the proposed model is already of appropriate size to fit our datasets and any regularization is taking away from model capacity.


% Finally, compared to the HAN-Flat model, we see an improvement of 0.87\% (News), 1.5\% (Yelp-L). The HAN model also captures phrase-level context like our model(due to the dot product attention), but unlike our model it does not make use of a bilinear projection for capturing fine-grained similarity between words and context-vector and the embedding is not structured; missing out on rich context especially for longer documents (as can be seen from improvements on News and Yelp-L datasets.)

% For the event detection task, we see that unstructured HAN model outperforms both HSA and our model whereas our model outperforms HSA by almost 1\%. The comparable performance of our model which is a multi-aspect model and the HAN model, which is a single aspect model can be attributed to the nature of the task, i.e. perhaps single attention is enough to capture the important keywords for event detection. Also learning multiple aspects might be unstable in hierarchical models which are deeper.
% Moreover, our model with context initialization as the mean of word embeddings outperforms our model with random initialization on all but MANSA dataset. This shows that this initialization method can be used as an effective technique to boost performance in models. 

% The proposed model outperforms the SA model ~\citep{lin2017structured} on all tasks by 
% 8.3\% (News), 5.9\% (Yelp), 13.7\% (Yelp Long) 6.7\% (IMDB) and 1.5\%  (MANSA). This improvement occurs with more than 70 times fewer parameters as demonstrated in section 3.3 (In section 3.3 we assume $l=d_a$, and $d_a=350$ but in our experiments $l=32$). The large improvement in Yelp Long can be explained by the ability of our model to attend to larger chunks of text as opposed to the SA model that forces attention only on a few words using the penalization term. Attending to larger chunks of text forms a more contextual document embedding that proves especially helpful in classifying longer reviews.

% Extrapolating the attention over larger chunks of text we get uniform attention to all words, which is equivalent to no attention or equal preference for all words which is what a simple LSTM model does (in a contextual setting and average of word embeddings in a non-contextual setting). We see that our model outperforms LSTM model by 2.9\% (News), 4.8\% (Yelp), 10.3\% (Yelp Long) and 1.14\% (IMDB). This improvement is lower as compared to the SA model which implies that these tasks prefer attention to larger chunks of text rather than smaller chunks but also tells us that attention is better than no-attention. Our model achieves this fine balance with regards to the attention structure.
% If we consider the non-contextual baseline of average of word embeddings we see an improvement of 2.3\% (News), 9.1\% (Yelp), 14.6\% (Yelp Long) and 3\% (IMDB) which proves that contextual dependencies captured by LSTM or CNN models are indeed important for the tasks.
% Compared to CNN models we see an improvement of 0.8\% (News), 1.5\% (Yelp), 4.3\% (Yelp Long), 3.4\% (IMDB) and finally, compared to the Flat HAN model, we see an improvement of 0.8\% (News), 1.6\% (Yelp Long), 1.02\% (IMDB) and 0.5\% (MANSA). 

% \begin{figure}[]
%  \centering
%  \begin{subfigure}{}{{\colorbox{MyBlue!210.7278}{good} \colorbox{MyBlue!218.6697}{service} \colorbox{MyBlue!32.8179}{and} \colorbox{MyBlue!186.5122}{very} \colorbox{MyBlue!189.8315}{clean} \colorbox{MyBlue!32.9187}{the} \colorbox{MyBlue!36.894}{only} \colorbox{MyBlue!126.5787}{thing} \colorbox{MyBlue!36.9184}{i} \colorbox{MyBlue!16.8599}{was} \colorbox{MyBlue!11.3368}{not} \colorbox{MyBlue!36.3602}{impressed} \colorbox{MyBlue!33.2507}{was} \colorbox{MyBlue!33.0884}{is} \colorbox{MyBlue!32.6035}{the} \colorbox{MyBlue!181.0751}{food} \colorbox{MyBlue!222.5592}{since} \colorbox{MyBlue!33.8856}{the} \colorbox{MyBlue!216.2462}{meat} \colorbox{MyBlue!174.305}{is} \colorbox{MyBlue!155.6017}{not} \colorbox{MyBlue!33.2453}{cooked} \colorbox{MyBlue!32.8041}{properly}}
%  \end{subfigure} \\
 
%  \begin{subfigure}{}{{\colorbox{MyPurple!38.0323}{good} \colorbox{MyPurple!36.5769}{service} \colorbox{MyPurple!41.5931}{and} \colorbox{MyPurple!91.8443}{very} \colorbox{MyPurple!90.5554}{clean} \colorbox{MyPurple!42.6902}{the} \colorbox{MyPurple!60.0232}{only} \colorbox{MyPurple!94.1897}{thing} \colorbox{MyPurple!60.0991}{i} \colorbox{MyPurple!87.7101}{was} \colorbox{MyPurple!114.3912}{not} \colorbox{MyPurple!120.39}{impressed} \colorbox{MyPurple!45.1843}{was} \colorbox{MyPurple!43.9938}{is} \colorbox{MyPurple!37.8634}{the} \colorbox{MyPurple!74.2687}{food} \colorbox{MyPurple!54.2422}{since} \colorbox{MyPurple!48.8177}{the} \colorbox{MyPurple!58.0863}{meat} \colorbox{MyPurple!77.3369}{is} \colorbox{MyPurple!104.6382}{not} \colorbox{MyPurple!45.0668}{cooked} \colorbox{MyPurple!33.2309}{properly}}
%   \end{subfigure} \\
  
%  \begin{subfigure}{}{{\colorbox{MyColor!100.0567}{good} \colorbox{MyColor!103.9471}{service} \colorbox{MyColor!38.1603}{and} \colorbox{MyColor!98.0883}{very} \colorbox{MyColor!99.0026}{clean} \colorbox{MyColor!38.2906}{the} \colorbox{MyColor!45.2236}{only} \colorbox{MyColor!86.0312}{thing} \colorbox{MyColor!45.3773}{i} \colorbox{MyColor!90.6674}{was} \colorbox{MyColor!97.8846}{not} \colorbox{MyColor!90.4352}{impressed} \colorbox{MyColor!39.4552}{was} \colorbox{MyColor!39.0777}{is}  \colorbox{MyColor!36.8009}{the} \colorbox{MyColor!97.2281}{food} \colorbox{MyColor!104.3188}{since} \colorbox{MyColor!40.3022}{the} \colorbox{MyColor!104.0032}{meat} \colorbox{MyColor!96.6652}{is} \colorbox{MyColor!93.2908}{not} \colorbox{MyColor!39.5829}{cooked} \colorbox{MyColor!35.5193}{properly}}
%  \end{subfigure}
%  \caption{An example review that illustrates the importance of multi-aspect attention. Here the customer is happy with the service but not happy with the food. Our model captures both of these aspects of the review in different attention distributions. Fig. shows visualizations of two distinct aspects (first two rows in green and purple) and the aggregate attention distribution over all aspects (last row in gray). The final distribution is aware of the both the aspects of the review.}
%   \label{fig:good}
% \end{figure}
% \begin{figure}

% \colorbox{MyBlue!210.7278}{good} \colorbox{MyBlue!218.6697}{service} \colorbox{MyBlue!32.8179}{and} \colorbox{MyBlue!186.5122}{very} \colorbox{MyBlue!189.8315}{clean} \colorbox{MyBlue!32.9187}{the} \colorbox{MyBlue!36.894}{only} \colorbox{MyBlue!126.5787}{thing} \colorbox{MyBlue!36.9184}{i} \colorbox{MyBlue!146.8599}{was} \colorbox{MyBlue!181.3368}{not} \colorbox{MyBlue!36.3602}{impressed} \colorbox{MyBlue!33.2507}{was} \colorbox{MyBlue!33.0884}{is} \colorbox{MyBlue!32.6035}{the} \colorbox{MyBlue!181.0751}{food} \colorbox{MyBlue!222.5592}{since} \colorbox{MyBlue!33.8856}{the} \colorbox{MyBlue!216.2462}{meat} \colorbox{MyBlue!174.305}{is} \colorbox{MyBlue!155.6017}{not} \colorbox{MyBlue!33.2453}{cooked} \colorbox{MyBlue!32.8041}{properly}
% \caption{(a)}
% \end{figure}
% \begin{figure}
% \colorbox{MyPurple!58.0323}{good} \colorbox{MyPurple!56.5769}{service} \colorbox{MyPurple!41.5931}{and} \colorbox{MyPurple!91.8443}{very} \colorbox{MyPurple!90.5554}{clean} \colorbox{MyPurple!42.6902}{the} \colorbox{MyPurple!60.0232}{only} \colorbox{MyPurple!94.1897}{thing} \colorbox{MyPurple!60.0991}{i} \colorbox{MyPurple!87.7101}{was} \colorbox{MyPurple!94.3912}{not} \colorbox{MyPurple!58.39}{impressed} \colorbox{MyPurple!45.1843}{was} \colorbox{MyPurple!43.9938}{is} \colorbox{MyPurple!37.8634}{the} \colorbox{MyPurple!74.2687}{food} \colorbox{MyPurple!54.2422}{since} \colorbox{MyPurple!48.8177}{the} \colorbox{MyPurple!58.0863}{meat} \colorbox{MyPurple!77.3369}{is} \colorbox{MyPurple!104.6382}{not} \colorbox{MyPurple!45.0668}{cooked} \colorbox{MyPurple!33.2309}{properly}
% \caption{(b)}
% \end{figure}
% \begin{figure}
% \colorbox{MyColor!100.0567}{good} \colorbox{MyColor!103.9471}{service} \colorbox{MyColor!38.1603}{and} \colorbox{MyColor!98.0883}{very} \colorbox{MyColor!99.0026}{clean} \colorbox{MyColor!38.2906}{the} \colorbox{MyColor!45.2236}{only} \colorbox{MyColor!86.0312}{thing} \colorbox{MyColor!45.3773}{i} \colorbox{MyColor!90.6674}{was} \colorbox{MyColor!97.8846}{not} \colorbox{MyColor!44.4352}{impressed} \colorbox{MyColor!39.4552}{was} \colorbox{MyColor!39.0777}{is} \colorbox{MyColor!36.8009}{the} \colorbox{MyColor!97.2281}{food} \colorbox{MyColor!104.3188}{since} \colorbox{MyColor!40.3022}{the} \colorbox{MyColor!104.0032}{meat} \colorbox{MyColor!96.6652}{is} \colorbox{MyColor!93.2908}{not} \colorbox{MyColor!39.5829}{cooked} \colorbox{MyColor!35.5193}{properly} \\
% \caption{An example of a review that illustrates the contextual usage of the word `good'. Here the customer is happy with the service but not happy with the food. Our model captures both of these aspects of the review in different attention distributions. Fig. shows the aggregate attention distribution assigned by our model over all aspects.}
%   \label{fig:good}
% \end{figure}
\subsection{Parameter vs Heads}
 In Transformer-based models attention layer can prove to be a memory bottleneck when resources are constrained. In this section, we compare the number of trainable parameters of the proposed model (LAMA) and  Transformer Encoder (TE). Table ~\ref{tab:param_vs_m} shows the increase in number of parameters (y-axis) when the number of attention heads are varied as 2, 4, 8, 16, 32, 64. Powers of 2 are picked because TE requires number of attention heads to be divisble by $d_{model}$ ~\citep{vaswani2017attention}. Note that reported parameters also contain GRU \& embedding parameters for LAMA and feed forward layer \& position embedding parameters for TE, although these parameters don't depend on number of attention heads. To ensure a fair comparison we pick BiGRU hidden dimension and $d_{model}$ both as 512. The hidden layer dimension of the final layer sentence classifier is 1024, which is the same for both models. It can be observed that the number of parameters in TE is constant for all heads which is consistent with its definition, because with increasing heads; Key, Value and Query projections parameters are scaled down. For LAMA, the number of parameters increases only slightly with increasing number of heads because \textbf{P} \& \textbf{Q} are the only parameter matrices that are dependent on the number of attention heads $m$ and for which the size increases (linearly). More importantly, it should be noted that for the number of heads for most practical use cases, the proposed model LAMA is almost 3 times more compact than Transformer Encoder. 
 
%  NOTE: Regularization is not helping - does that mean that our model is already at its optimal capacity? i.e. there is no fear of overparamterization.
%  However we show that multiple heads do carry benefit in \S\ref{sec:why_multi}.
% In the second scenario we vary the number of encoder layers of the TE model from 1 to 4 and compare the performance of TE vs our model. We analyse the number of parameters in the each model needed to reach the respective performance. 

\begin{table}[]
 \caption{Comparison of number of trainable parameters in the attention layer of LAMA and TE with increasing number of attention heads. Number of parameters increase linearly for LAMA whereas for TE they are constant. Overall LAMA is more parameter efficient than TE.}
 \centering
\begin{tabular}{@{}lll@{}}
\toprule
\# heads & \begin{tabular}[c]{@{}l@{}}\# parameters (LAMA)\\    (in millions)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\# parameters (TE)\\    (in millions)\end{tabular} \\ \midrule
2        & 6.403                                                                           & 18.465                                                                        \\
4        & 6.405                                                                           & 18.465                                                                        \\
8        & 6.409                                                                           & 18.465                                                                        \\
16       & 6.418                                                                           & 18.465                                                                        \\
32       & 6.434                                                                           & 18.465                                                                        \\
64       & 6.468                                                                           & 18.465                                                                        \\
% 128      & 6.536                                                                           & 18.465                                                                        \\ 
\bottomrule
\end{tabular}
 \label{tab:param_vs_m}
\end{table}
% \begin{figure}[ht!]
%  \centering
%   \includegraphics[height=.20\textheight
%   ]{images/heads_vs_params.pdf}
%  \caption{Comparison of number of trainable parameters in the attention layer of SAN, LAMA and TE with increasing number of attention heads. Number of parameters increase linearly for SAN and LAMA whereas for TE they increase exponentially w.r.t the number of heads. Number of parameters in SAN exceeds the number of parameters in LAMA by a constant.}
%  \label{fig:param_vs_m}
% \vspace{-1em}
% \end{figure}

% \begin{figure}[ht!]
%  \centering
%   \includegraphics[height=.15\textheight
%   ]{images/loss_vs_epochs.pdf}
%  \caption{Figure shows the train loss w.r.t. the number of epochs for the Reuters and the News datasets for  TE and LAMA models.}
%  \label{fig:acc_vs_epoch}
% \vspace*{-0.2in}
% \end{figure}

\subsection{Runtime} 
It should be noted that since LAMA is applied on top of RNN the computation is sequential and attention cannot be computed unless all RNN hidden states are available. Hence, the computational time increases linearly with input length and quadratically with hidden state dimension $(O(n*h^2))$. Once RNN hidden states are available the complexity of the attention layer LAMA is $O(n*m*h)$. In comparison, the complexity of the self-attention mechanism in Transformer is $O(n^2*d)$, where $d$ is the hidden state dimension. It increases quadratically with increasing input length and linearly with hidden state dimension. In this section, we compare the runtimes of LAMA and a 1-layer Transformer Encoder. For a fair comparison we compare the runtimes of LAMA free from RNN. We propose, LAMA Encoder -- a model that doesn't use RNN to model sequential dependencies and directly operates on the word embeddings of the inputs. That is, the hidden state matrix $\textbf{H}$ in Eq. ~\ref{eq:attn} is populated by the pretrained word embeddings.  Fig ~\ref{fig:time_vs_len} shows the  average runtime per epoch (averaged over 10 epochs) of LAMA Encoder (LE) and Transformer Encoder (TE) when sequence lengths are increased from 50 to 250 for IMDB and Reuters datasets. It can be seen from the figure that TE is computationally more expensive per epoch than LE.
LE is also a competitive model with test accuracies of 83.0 \%  on IMDB and 93.9\% on Reuters as compared to 81.7\% (IMDB) and 90.1\% (REUTERS) of TE.

% However operations are parallelizable on GPU. But in case of Transformer Encoder, CPU usage and GPU usage is much larger than LSTM as can be seen in Fig ~\ref{fig:time_vs_len}.



\begin{figure*}
 \centering
   \includegraphics[width=0.7\textwidth]{images/time_vs_len.pdf}
 \caption{\small{Figure shows the average run time per epoch in seconds (averaged over 10 epochs) for LAMA Encoder (LE) and Transformer Encoder (TE) models as a function of input sequence length (50 to 250). It can be seen that TE (green) is more computationally expensive compared to LAMA (blue). LE is LAMA attention mechanism applied directly to word embeddings without computing GRU hidden states. } }
 \label{fig:time_vs_len}
%  \vspace*{-0.2in}
 \end{figure*}
% In table ~\ref{tab:complexity} we saw that complexity of LAMA scales linearly whereas complexity of TE scales quadratically with input length. In this section, we analyse the average train time of the different models with increasing input length.  We report average training time over 10 epochs for both the models with increasing input length. We pick the hyperparameters corresponding to the best model and report the performance on IMDB and News datasets. 

% Moreover, it should be noted thatIn the results section we already saw the training times for BERT per epoch. 

% We observe that for LAMA most of CPU time (46 \%) and GPU time (46\%)  is attributed to the RNN operation whereas for the Transformer Encoder the most expensive operation for both CPU and GPU is the matrix multiplication operation coming from the self-attention layer (96 \%). 

% This is also one of the main reasons why the proposed model is faster than TE. Since LAMA is RNN based there is a clear relationship between compute time and input length, because RNN operation is sequential. For TE there is no such clear relationship because self-attention operation is not sequential in that case ~\citep{vaswani2017attention}. 
% However, clearly even including the RNN-time LAMA is  much faster than TE.

~\subsection{Parameters vs Accuracy}
On the YELP-P dataset our model is outperformed by BERT by 1.8 \%. However it it worth noting the cost of this performance improvement. Fig. ~\ref{fig:perf_vs_params} shows the accuracy of different models and their  corresponding parameters on the YELP-P dataset. It can be seen that \textsf{LAMA+ctx} outperforms SAN \& TE with fewer parameters (difference being linear). BERT slightly outperforms \textsf{LAMA+ctx} however with more than an order of magnitude increase in parameters.
% In this section we plot the number of parameters vs the performance of the models CNN, BiGRU, SAN, TE and . 
\begin{figure}
 \centering
   \includegraphics[width=0.45\textwidth]{images/params_vs_acc_scatter.pdf}
 \caption{\small{Figure shows the accuracy (y-axis) of the models LAMA, SAN, TE and BERT models on YELP-P dataset when viewed against the model parameters (x-axis). LAMA outperforms SAN and TE while also being more parameter efficient. BERT outperforms LAMA by 1.8\% but by more than an order of magnitude increase in parameters.} }
 \label{fig:perf_vs_params}
%  \vspace*{-0.2in}
 \end{figure}
% \subsection{Convergence Analysis}
% In this section we analyse the run time of one epoch for each of the model.
% We plot the training loss per epoch for the three attention-based models (SAN, TE and LAMA). As can be seen from Fig. ~\ref{fig:acc_vs_epoch} on an average LAMA converges faster than SAN and TE and to a smaller optimum.
% We plot the training loss per epoch for the three attention-based models (SAN, TE and LAMA). As can be seen from Fig. ~\ref{fig:acc_vs_epoch} on an average LAMA converges faster than SAN and TE and to a smaller optimum.
% TODO: Number of transformer layers


\subsection{Contextual Attention Weights}
% To validate that our model picks up important words while computing the sentence embedding we perform an analysis similar to prior approches ~\citep{han}. If words were inherently not important then models without attention such as LSTMs that also capture contextual dependencies might work well. However, the importance of words is highly context dependent and models such as LSTMs aren't good enough to capture those long term dependencies. For instance, the word `good' may appear in a review that has the lowest rating either because users are only happy with part of the service or because they use it in a negation, such as not good. See example in Figure ~\ref{fig:probs_amazing}.

To verify that our model captures context dependent word importance and is interpretable we peform qualitative analysis.  We plot the distribution of the attention weights of the positive words `amazing', `happy' and `recommended' and negative words `poor', `terrible' and `worst' from the test split of the Yelp data set as shown in Figure \ref{fig:probs_amazing}. We plot the distribution when conditioned on the ratings of the reviews from 1 to 5. It can be seen from Figure ~\ref{fig:probs_amazing} that the weight of positive words concentrates on the low end in the reviews with rating 1 (blue curve). As the rating increases, the weight distribution shifts to the right. This indicates that positive words play a more important role for reviews with higher ratings. The trend is opposite for the negative words where words with negative connotation have lower attention weights for reviews with rating 5 (purple curve). However, there are a few exceptions. For example, it is intuitive that `amazing' gets a high weight for reviews with high ratings but it also gets a high weight for reviews with rating 2 (orange curve). This is because, inspecting the Yelp dataset we find that `amazing' occurs quite frequently with the word `not' in the reviews with rating 2; `above average but not amazing', `was ok but not amazing'. Our model captures this phrase-level context and assigns similar weights to `not' and `amazing'. `not' being a negative word gets a high weight for lower ratings and hence so does `amazing'. 
Similarly, other exceptions such as `terrible' for rating 4 can be explained due to the fact that customers might dislike one aspect of a business such as their service but like another aspect such as food.

% This confirms that our model can capture nuanced context-dependent word importance.
\begin{table}[]
\centering
\caption{\small{Top attended words for Yelp dataset from reviews with ratings 1 and 5 (indicated in paratheses) and Reuters(r8) Dataset.}}
\label{tab:kw}
% \small
\begin{tabular}{@{}llll@{}}
\toprule
Yelp(1) & Yelp(5)  & r8(ship)& r8(money) \\ \midrule
\begin{tabular}[c]{@{}l@{}}inconsiderate \\ rudest \\ goodnight \\ worst\\ ever\\ boycott\\ loud\\ livid\\ some\\  hassle\\  friendly \\ ugh \\ dealership\\ brutal \\ rather \\ 1 \\ pizza\\ slow \\ torture \\ absolute\end{tabular} & \begin{tabular}[c]{@{}l@{}}recommend \\ trust\\ referred \\ downside\\  professional\\  100\\  happy\\ attentive\\  stars \\ please \\ delicious \\ safe\\ worth\\ very\\ would \\ blown\\  sensitive \\ removed\\ impressed \\ looks\end{tabular} & \begin{tabular}[c]{@{}l@{}}kuwait \\ gulf \\ south\\ tanker \\ cargo\\ warships \\ pentagon \\ says \\ begin \\ iranian \\ shipping \\ from\\ demand \\ salvage \\ trade \\ production \\ japan \\ gulf \\ india\\  combat\end{tabular} & \begin{tabular}[c]{@{}l@{}}currencies\\ monetary\\ miyazawa \\ stoltenberg\\ accord \\ louvre \\ fed \\ cooperation\\  rate \\ poehl\\ exchange\\ stability \\ currency \\ german \\ reagan \\ pact \\ policy \\support \\trade\\deficit\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}
To further illustrate context-dependent word importance Table ~\ref{tab:kw} lists top attended keywords for Yelp and Reuters datasets. 
% It can be seen that certain words that often occur in pairs such as `would recommend', `very professional', `very delicious' appear in the list for Yelp and `exchange rate', `trade deficit' for Reuters. This is because the model assigns close attention weights to the words in these phrases because they occur frequently together.
Note that superlatives such `100 stars' appear in the list which are strong indicators of the sentiment of a review.

\begin{figure}[!t]
 \centering
  \includegraphics[width=0.5\textwidth]{images/word_probs.pdf} \caption{\small{Attention weight ($x$-$axis$) distribution of the positive words `amazing', `happy' \& `recommend' and negative words `poor', `terrible', \& `worst'. Positive words tend to get higher weights in reviews with higher ratings (3-5) whereas negative words get higher weights for lower ratings (1-2)} Example `terrible' and `poor' get a very low weight for reviews with ratings 5 and `recommend' and `amazing' get high attention weights for reviews with ratings 4 and 5.}
 \label{fig:probs_amazing}
%  \vspace*{-0.2in}
 \end{figure}
% To verify that our model can capture context dependent word importance, we plot the distribution of the attention weights of the the positive word `amazing' and the negative word `bad' from the test split of the Yelp data set as shown in Figures \ref{fig:probs_amazing} \& \ref{fig:probs_bad} ($a-f$). We plot the distribution when conditioned on the ratings of the review. Subfigures $(b)-(f)$ in Figure ~\ref{fig:probs_amazing} and Figure ~\ref{fig:probs_bad} correspond
% to the rating 1-5 respectively. In particular, Figure ~\ref{fig:probs_amazing}(b) shows that the weight of `amazing' concentrates on the low end in the reviews with rating 1. As the rating increases the weight distribution shifts to the right although not a stark shift because our model  attends to chunks of words and does not rely on only specific words. This means that the word amazing plays a more important role for reviews with higher ratings. The trend is opposite for the word bad as can be seen from  Figure ~\ref{fig:probs_bad}. This confirms that our model can capture the context-dependent word importance. Note that the average number of tokens in this dataset is 216 and hence for a uniform distribution each token gets a weight of 0.005. Hence, the low attention weights such as 0.01 in the Figure should not be misconstrued as they are almost 50\% greater than uniform weights. 

% \begin{figure}[t!]
%  \centering
%   \includegraphics[width=0.47\textwidth]{images/probs_amazing.pdf}
%  \caption{\small{Attention weight distribution of the word `amazing'. (a) aggregate distribution on the test split; (b)-(f) for reviews with ratings 1-5 respectively. We can see that the weight distribution shifts to higher end as the rating goes higher.}}
%  \label{fig:probs_amazing}
%  \vspace*{-0.2in}
%  \end{figure}

% \begin{figure}[t!]
%  \centering
%   \includegraphics[width=0.47\textwidth]{images/probs_bad.pdf}
%  \caption{\small{Attention weight distribution of the word bad. The setup is as above: (a) contains the aggregate distribution, while (b)-(f) contain 
%  stratifications to reviews with ratings 1-5 respectively. Contrary to before, the word bad is considered important for poor ratings and less so for good ones.}}
%  \label{fig:probs_bad}
%  \vspace*{-0.2in}
%  \end{figure}

\subsection{Why Multiple Heads}
\label{sec:why_multi}
\begin{figure}[H]
%  \centering
   \includegraphics[width=0.5\textwidth]{images/acc_vs_heads.pdf}
%   \subfigure{\includegraphics[width=0.49\columnwidth]{images/accuracy_vs_hops.pdf}}
%   \subfigure{\includegraphics[width=0.49\columnwidth]{images/acc_vs_hops_imdb.pdf}}
 \caption{\small{Figure shows the effect of using multiple attention heads. Validation accuracy of \textsf{LAMA+Ctx} is plotted for different values of $m$ for the Yelp-L dataset(left) and the IMDB dataset(right). $x$-$axis$ indicates the number of epochs, $y$-$axis$ indicates the accuracy. Accuracy peaks at $m=15$ for both Yelp-L and IMDB. } }
 \label{fig:acc}
%  \vspace*{-0.2in}
 \end{figure}

Previous works have shown that more heads does not necessarily lead to better performance for machine translation tasks ~\citep{michel2019sixteen}. In this analysis, we seek to answer a similar question for text classification. 

We evaluate the model performance as we vary the number of attention heads $m$ from 1 to 25.  Specifically, we plot the validation accuracy vs. epochs for different values of $m$, for the Yelp-L and IMDB datasets. We vary $m$ from 1 to 20 to get 5 models with $m=1$, $m=5$, $m=10$, $m=15$ and $m=20$. The plots are shown in Figure ~\ref{fig:acc}. From the figure we can see that for the Yelp-L dataset model performance peaks for $m=15$ and then starts falling for $m=20$. We can clearly see a significant difference between $m=1$ and $m=20$, showing that having a multi-aspect attention mechanism helps. For the IMDB dataset model with $m=15$ performs the best whereas model with $m=1$ performs the worst although performances for $m=5,15,20$ are similar.

% \subsection{Visualization}
% In order to provide qualitative examples we visualize the attention distributions for  example reviews from the Yelp Dataset. Fig ~\ref{fig:good} shows the importance of using multi-aspect attention. In this example the customer is happy with the service but not happy with the food. Our model captures both of these aspects of the review in different attention distributions. The final distribution is aware of the both the aspects of the review. Further, in Table ~\ref{tab:viz} we plot 3 aspects of a review and each row visualizes a different aspect. Darker shades represent higher attention weights. As can be seen from the table aspect 2 tries to learn highly positive sentiment keywords such as `pretty excited', `definitely' and `delicious'. For aspect 3, although it pays attention to some positive words such as `amazing' and  `fantastic' negative words such as `not attentive', `forgotten and `failed' are also highlighted. This aspect seems to learn the negative sentiment in the review. From the review looks like the customer was happy with the food but not the service as captured by two aspects by our model and correctly assigning it a rating of 3. 
% \begin{table*}[]
% \small
% \caption{Table shows visualization of three different aspects for an example review from the Yelp Dataset. Each row represents a different aspects. Darker shades represent higher attention weights. }
% \begin{tabular}{|l|}

% \hline
% \colorbox{MyColor!38.0144}{We} \colorbox{MyColor!38.2521}{were} \colorbox{MyColor!36.7891}{pretty} \colorbox{MyColor!37.7362}{excited} \colorbox{MyColor!40.7745}{to} \colorbox{MyColor!39.9491}{come} \colorbox{MyColor!39.9184}{here}  \colorbox{MyColor!38.8898}{while} \colorbox{MyColor!40.81}{on} \colorbox{MyColor!37.6746}{vacation} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!80.617}{The} \colorbox{MyColor!79.4324}{experience} \colorbox{MyColor!36.9799}{began} \colorbox{MyColor!37.7101}{great} \colorbox{MyColor!36.7976}{but} \colorbox{MyColor!38.1722}{went} \colorbox{MyColor!34.5055}{south}\colorbox{MyColor!10.0}{.} \colorbox{MyColor!39.6386}{As} \colorbox{MyColor!39.9392}{far} \colorbox{MyColor!38.4074}{as} \\ \colorbox{MyColor!40.3307}{the} \colorbox{MyColor!37.7573}{service}  \colorbox{MyColor!39.0651}{goes} \colorbox{MyColor!40.2697}{it} \colorbox{MyColor!34.9239}{felt} \colorbox{MyColor!39.3041}{as} \colorbox{MyColor!35.2448}{though} \colorbox{MyColor!40.2694}{we} \colorbox{MyColor!40.005}{were} \colorbox{MyColor!38.3608}{forgotten} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!38.5068}{Waiter} \colorbox{MyColor!40.2643}{was} \colorbox{MyColor!40.7667}{not} \colorbox{MyColor!40.8062}{very}  \colorbox{MyColor!36.2722}{attentive} \colorbox{MyColor!40.9236}{and} \colorbox{MyColor!70.9257}{they} \colorbox{MyColor!78.7271}{failed} \colorbox{MyColor!71.1925}{to} \colorbox{MyColor!70.7952}{put} \colorbox{MyColor!70.9959}{our} \\ \colorbox{MyColor!71.0686}{order} \colorbox{MyColor!71.0958}{in} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!71.0398}{ended} \colorbox{MyColor!70.4264}{up}   \colorbox{MyColor!70.6465}{being} \colorbox{MyColor!70.7631}{there} \colorbox{MyColor!70.5397}{for} \colorbox{MyColor!70.903}{almost} \colorbox{MyColor!71.0487}{2} \colorbox{MyColor!68.3065}{hours} \colorbox{MyColor!39.763}{because}  \colorbox{MyColor!39.9156}{of} \colorbox{MyColor!37.5174}{this} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!36.5458}{good} \colorbox{MyColor!37.3198}{was} \colorbox{MyColor!37.1626}{amazing} \colorbox{MyColor!39.9682}{and} \colorbox{MyColor!35.9224}{fantastic} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!38.1096}{As} \colorbox{MyColor!39.1414}{far} \\ \colorbox{MyColor!38.0486}{as} \colorbox{MyColor!39.5777}{the}  \colorbox{MyColor!38.178}{brunch} \colorbox{MyColor!38.6565}{goes}  \colorbox{MyColor!36.0191}{though}  \colorbox{MyColor!40.3345}{i} \colorbox{MyColor!37.7996}{would}  \colorbox{MyColor!36.9689}{definitely} \colorbox{MyColor!35.9743}{give} \colorbox{MyColor!36.6471}{hash} \colorbox{MyColor!35.2991}{another} \colorbox{MyColor!35.4868}{show} \colorbox{MyColor!37.9068}{because} \colorbox{MyColor!39.7444}{the} \colorbox{MyColor!34.3956}{food} \colorbox{MyColor!36.6979}{was} \colorbox{MyColor!36.3883}{delicious} \colorbox{MyColor!10.0}{.} \\ \hline

% \colorbox{MyColor!63.3105}{We} \colorbox{MyColor!69.5629}{were} \colorbox{MyColor!189.2819}{pretty} \colorbox{MyColor!204.0624}{excited} \colorbox{MyColor!27.879}{to} \colorbox{MyColor!28.3116}{come} \colorbox{MyColor!27.9682}{here} \colorbox{MyColor!27.9411}{while} \colorbox{MyColor!27.9298}{on} \colorbox{MyColor!41.7407}{vacation} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!27.8703}{The} \colorbox{MyColor!33.2327}{experience} \colorbox{MyColor!173.5128}{began} \colorbox{MyColor!42.1715}{great} \colorbox{MyColor!61.3915}{but} \colorbox{MyColor!65.4224}{went} \colorbox{MyColor!103.4963}{south} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!28.2256}{As} \colorbox{MyColor!27.8603}{far}  \colorbox{MyColor!30.1969}{as} \\ \colorbox{MyColor!28.0113}{the} \colorbox{MyColor!122.9294}{service} \colorbox{MyColor!37.3099}{goes} \colorbox{MyColor!27.9306}{it} \colorbox{MyColor!71.8799}{felt} \colorbox{MyColor!27.9729}{as} \colorbox{MyColor!86.5476}{though} \colorbox{MyColor!32.1715}{we} \colorbox{MyColor!38.2283}{were} \colorbox{MyColor!90.0869}{forgotten} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!110.3746}{Waiter} \colorbox{MyColor!38.0688}{was} \colorbox{MyColor!44.503}{not} \colorbox{MyColor!28.9436}{very} \colorbox{MyColor!59.7754}{attentive} \colorbox{MyColor!27.9149}{and} \colorbox{MyColor!30.4378}{they} \colorbox{MyColor!139.2929}{failed} \colorbox{MyColor!28.0517}{to} \colorbox{MyColor!32.2755}{put} \colorbox{MyColor!28.0125}{our} \\ 
% \colorbox{MyColor!29.0591}{order} \colorbox{MyColor!27.9069}{in} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!27.988}{ended} \colorbox{MyColor!28.2549}{up} \colorbox{MyColor!27.8768}{being} \colorbox{MyColor!27.8719}{there} \colorbox{MyColor!27.9071}{for} \colorbox{MyColor!28.2161}{almost} \colorbox{MyColor!28.5044}{2} \colorbox{MyColor!66.2699}{hours} \colorbox{MyColor!27.9886}{because} \colorbox{MyColor!29.5496}{of} \colorbox{MyColor!116.8055}{this} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!45.325}{good} \colorbox{MyColor!126.8181}{was} \colorbox{MyColor!112.2109}{amazing} \colorbox{MyColor!28.5598}{and} \colorbox{MyColor!84.4563}{fantastic} \colorbox{MyColor!27.931}{as} \colorbox{MyColor!28.4084}{far} \\ \colorbox{MyColor!27.9586}{as} \colorbox{MyColor!27.8638}{the} \colorbox{MyColor!33.2428}{brunch} \colorbox{MyColor!37.8696}{goes} \colorbox{MyColor!62.2716}{though} \colorbox{MyColor!27.9914}{i} \colorbox{MyColor!68.461}{would} \colorbox{MyColor!184.5746}{definitely} \colorbox{MyColor!194.9537}{give} \colorbox{MyColor!195.4749}{hash} \colorbox{MyColor!92.8419}{another} \colorbox{MyColor!191.3169}{show} \colorbox{MyColor!28.2446}{because} \colorbox{MyColor!27.862}{the} \colorbox{MyColor!155.8021}{food} \colorbox{MyColor!167.1557}{was} \colorbox{MyColor!190.4349}{delicious} \colorbox{MyColor!10.0}{.} \\ \hline 

% \colorbox{MyColor!85.7879}{We} \colorbox{MyColor!86.8925}{were} \colorbox{MyColor!47.6183}{pretty} \colorbox{MyColor!36.3039}{excited} \colorbox{MyColor!32.8496}{to} \colorbox{MyColor!38.3773}{come} \colorbox{MyColor!29.3936}{here} \colorbox{MyColor!34.6001}{while} \colorbox{MyColor!34.2268}{on} \colorbox{MyColor!121.5652}{vacation}  \colorbox{MyColor!10.0}{.} \colorbox{MyColor!31.724}{The} \colorbox{MyColor!56.5994}{experience} \colorbox{MyColor!55.9174}{began} \colorbox{MyColor!122.1099}{great} \colorbox{MyColor!135.107}{but} \colorbox{MyColor!136.2672}{went} \colorbox{MyColor!132.183}{south} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!27.319}{As} \colorbox{MyColor!31.9143}{far} \colorbox{MyColor!21.6847}{as} \\ \colorbox{MyColor!28.9698}{the} \colorbox{MyColor!126.8933}{service} \colorbox{MyColor!115.0441}{goes} \colorbox{MyColor!34.4115}{it} \colorbox{MyColor!136.4623}{felt} \colorbox{MyColor!35.1309}{as} \colorbox{MyColor!135.8982}{though} \colorbox{MyColor!53.8069}{we} \colorbox{MyColor!66.5958}{were} \colorbox{MyColor!135.8994}{forgotten} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!131.0263}{Waiter} \colorbox{MyColor!66.3253}{was} \colorbox{MyColor!124.8363}{not} \colorbox{MyColor!42.1331}{very} \colorbox{MyColor!134.4877}{attentive} \colorbox{MyColor!33.8659}{and} \colorbox{MyColor!48.367}{they} \colorbox{MyColor!120.9087}{failed} \colorbox{MyColor!35.8341}{to} \colorbox{MyColor!54.0606}{put} \colorbox{MyColor!35.4217}{our} \\ \colorbox{MyColor!42.6813}{order} \colorbox{MyColor!30.6969}{in} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!35.0803}{Ended} \colorbox{MyColor!27.1882}{up} \colorbox{MyColor!32.868}{being} \colorbox{MyColor!32.3232}{there} \colorbox{MyColor!33.8647}{for} \colorbox{MyColor!37.504}{almost} \colorbox{MyColor!39.5842}{2} \colorbox{MyColor!86.4346}{hours} \colorbox{MyColor!35.3435}{because} \colorbox{MyColor!45.0118}{of} \colorbox{MyColor!78.9261}{this} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!75.4464}{good} \colorbox{MyColor!75.467}{was} \colorbox{MyColor!130.332}{amazing} \colorbox{MyColor!40.0523}{and} \colorbox{MyColor!136.3328}{fantastic} \colorbox{MyColor!34.1459}{as} \colorbox{MyColor!39.0689}{far} \\ \colorbox{MyColor!34.6088}{as} \colorbox{MyColor!31.4786}{the} \colorbox{MyColor!56.5627}{brunch} \colorbox{MyColor!65.985}{goes} \colorbox{MyColor!135.2044}{though} \colorbox{MyColor!35.3142}{i} \colorbox{MyColor!136.7223}{would} \colorbox{MyColor!50.2985}{definitely} \colorbox{MyColor!43.8164}{give} \colorbox{MyColor!43.6829}{hash} \colorbox{MyColor!134.8802}{another} \colorbox{MyColor!45.9909}{show} \colorbox{MyColor!37.6619}{because} \colorbox{MyColor!31.6226}{the} \colorbox{MyColor!63.25}{food} \colorbox{MyColor!58.8528}{was} \colorbox{MyColor!46.8313}{delicious} \colorbox{MyColor!10.0}{.} \\ \hline
% \end{tabular}
% \label{tab:viz}
% \end{table*}





% \begin{table*}[]
% \small
% \caption{Table shows visualization of three different aspects for an example review from the Yelp Dataset. Each row represents a different aspects. Darker shades represent higher attention weights. }
% \begin{tabular}{|l|}

% \hline
% \colorbox{MyColor!38.0144}{We} \colorbox{MyColor!38.2521}{were} \colorbox{MyColor!36.7891}{pretty} \colorbox{MyColor!37.7362}{excited} \colorbox{MyColor!40.7745}{to} \colorbox{MyColor!39.9491}{come} \colorbox{MyColor!39.9184}{here}  \colorbox{MyColor!38.8898}{while} \colorbox{MyColor!40.81}{on} \colorbox{MyColor!37.6746}{vacation} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!80.617}{The} \colorbox{MyColor!79.4324}{experience} \colorbox{MyColor!36.9799}{began} \colorbox{MyColor!37.7101}{great} \colorbox{MyColor!36.7976}{but} \colorbox{MyColor!38.1722}{went} \colorbox{MyColor!34.5055}{south}\colorbox{MyColor!10.0}{.} \colorbox{MyColor!39.6386}{As} \colorbox{MyColor!39.9392}{far} \colorbox{MyColor!38.4074}{as} \\ \colorbox{MyColor!40.3307}{the} \colorbox{MyColor!37.7573}{service}  \colorbox{MyColor!39.0651}{goes} \colorbox{MyColor!40.2697}{it} \colorbox{MyColor!34.9239}{felt} \colorbox{MyColor!39.3041}{as} \colorbox{MyColor!35.2448}{though} \colorbox{MyColor!40.2694}{we} \colorbox{MyColor!40.005}{were} \colorbox{MyColor!38.3608}{forgotten} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!38.5068}{Waiter} \colorbox{MyColor!40.2643}{was} \colorbox{MyColor!40.7667}{not} \colorbox{MyColor!40.8062}{very}  \colorbox{MyColor!36.2722}{attentive} \colorbox{MyColor!40.9236}{and} \colorbox{MyColor!70.9257}{they} \colorbox{MyColor!78.7271}{failed} \colorbox{MyColor!71.1925}{to} \colorbox{MyColor!70.7952}{put} \colorbox{MyColor!70.9959}{our} \\ \colorbox{MyColor!71.0686}{order} \colorbox{MyColor!71.0958}{in} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!71.0398}{ended} \colorbox{MyColor!70.4264}{up}   \colorbox{MyColor!70.6465}{being} \colorbox{MyColor!70.7631}{there} \colorbox{MyColor!70.5397}{for} \colorbox{MyColor!70.903}{almost} \colorbox{MyColor!71.0487}{2} \colorbox{MyColor!68.3065}{hours} \colorbox{MyColor!39.763}{because}  \colorbox{MyColor!39.9156}{of} \colorbox{MyColor!37.5174}{this} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!36.5458}{good} \colorbox{MyColor!37.3198}{was} \colorbox{MyColor!37.1626}{amazing} \colorbox{MyColor!39.9682}{and} \colorbox{MyColor!35.9224}{fantastic} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!38.1096}{As} \colorbox{MyColor!39.1414}{far} \\ \colorbox{MyColor!38.0486}{as} \colorbox{MyColor!39.5777}{the}  \colorbox{MyColor!38.178}{brunch} \colorbox{MyColor!38.6565}{goes}  \colorbox{MyColor!36.0191}{though}  \colorbox{MyColor!40.3345}{i} \colorbox{MyColor!37.7996}{would}  \colorbox{MyColor!36.9689}{definitely} \colorbox{MyColor!35.9743}{give} \colorbox{MyColor!36.6471}{hash} \colorbox{MyColor!35.2991}{another} \colorbox{MyColor!35.4868}{show} \colorbox{MyColor!37.9068}{because} \colorbox{MyColor!39.7444}{the} \colorbox{MyColor!34.3956}{food} \colorbox{MyColor!36.6979}{was} \colorbox{MyColor!36.3883}{delicious} \colorbox{MyColor!10.0}{.} \\ \hline

% \colorbox{MyColor!63.3105}{We} \colorbox{MyColor!69.5629}{were} \colorbox{MyColor!189.2819}{pretty} \colorbox{MyColor!204.0624}{excited} \colorbox{MyColor!27.879}{to} \colorbox{MyColor!28.3116}{come} \colorbox{MyColor!27.9682}{here} \colorbox{MyColor!27.9411}{while} \colorbox{MyColor!27.9298}{on} \colorbox{MyColor!41.7407}{vacation} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!27.8703}{The} \colorbox{MyColor!33.2327}{experience} \colorbox{MyColor!173.5128}{began} \colorbox{MyColor!42.1715}{great} \colorbox{MyColor!61.3915}{but} \colorbox{MyColor!65.4224}{went} \colorbox{MyColor!103.4963}{south} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!28.2256}{As} \colorbox{MyColor!27.8603}{far}  \colorbox{MyColor!30.1969}{as} \\ \colorbox{MyColor!28.0113}{the} \colorbox{MyColor!122.9294}{service} \colorbox{MyColor!37.3099}{goes} \colorbox{MyColor!27.9306}{it} \colorbox{MyColor!71.8799}{felt} \colorbox{MyColor!27.9729}{as} \colorbox{MyColor!86.5476}{though} \colorbox{MyColor!32.1715}{we} \colorbox{MyColor!38.2283}{were} \colorbox{MyColor!90.0869}{forgotten} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!110.3746}{Waiter} \colorbox{MyColor!38.0688}{was} \colorbox{MyColor!44.503}{not} \colorbox{MyColor!28.9436}{very} \colorbox{MyColor!59.7754}{attentive} \colorbox{MyColor!27.9149}{and} \colorbox{MyColor!30.4378}{they} \colorbox{MyColor!139.2929}{failed} \colorbox{MyColor!28.0517}{to} \colorbox{MyColor!32.2755}{put} \colorbox{MyColor!28.0125}{our} \\ 
% \colorbox{MyColor!29.0591}{order} \colorbox{MyColor!27.9069}{in} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!27.988}{ended} \colorbox{MyColor!28.2549}{up} \colorbox{MyColor!27.8768}{being} \colorbox{MyColor!27.8719}{there} \colorbox{MyColor!27.9071}{for} \colorbox{MyColor!28.2161}{almost} \colorbox{MyColor!28.5044}{2} \colorbox{MyColor!66.2699}{hours} \colorbox{MyColor!27.9886}{because} \colorbox{MyColor!29.5496}{of} \colorbox{MyColor!116.8055}{this} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!45.325}{good} \colorbox{MyColor!126.8181}{was} \colorbox{MyColor!112.2109}{amazing} \colorbox{MyColor!28.5598}{and} \colorbox{MyColor!84.4563}{fantastic} \colorbox{MyColor!27.931}{as} \colorbox{MyColor!28.4084}{far} \\ \colorbox{MyColor!27.9586}{as} \colorbox{MyColor!27.8638}{the} \colorbox{MyColor!33.2428}{brunch} \colorbox{MyColor!37.8696}{goes} \colorbox{MyColor!62.2716}{though} \colorbox{MyColor!27.9914}{i} \colorbox{MyColor!68.461}{would} \colorbox{MyColor!184.5746}{definitely} \colorbox{MyColor!194.9537}{give} \colorbox{MyColor!195.4749}{hash} \colorbox{MyColor!92.8419}{another} \colorbox{MyColor!191.3169}{show} \colorbox{MyColor!28.2446}{because} \colorbox{MyColor!27.862}{the} \colorbox{MyColor!155.8021}{food} \colorbox{MyColor!167.1557}{was} \colorbox{MyColor!190.4349}{delicious} \colorbox{MyColor!10.0}{.} \\ \hline 

% \colorbox{MyColor!85.7879}{We} \colorbox{MyColor!86.8925}{were} \colorbox{MyColor!47.6183}{pretty} \colorbox{MyColor!36.3039}{excitepd} \colorbox{MyColor!32.8496}{to} \colorbox{MyColor!38.3773}{come} \colorbox{MyColor!29.3936}{here} \colorbox{MyColor!34.6001}{while} \colorbox{MyColor!34.2268}{on} \colorbox{MyColor!121.5652}{vacation}  \colorbox{MyColor!10.0}{.} \colorbox{MyColor!31.724}{The} \colorbox{MyColor!56.5994}{experience} \colorbox{MyColor!55.9174}{began} \colorbox{MyColor!122.1099}{great} \colorbox{MyColor!135.107}{but} \colorbox{MyColor!136.2672}{went} \colorbox{MyColor!132.183}{south} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!27.319}{As} \colorbox{MyColor!31.9143}{far} \colorbox{MyColor!21.6847}{as} \\ \colorbox{MyColor!28.9698}{the} \colorbox{MyColor!126.8933}{service} \colorbox{MyColor!115.0441}{goes} \colorbox{MyColor!34.4115}{it} \colorbox{MyColor!136.4623}{felt} \colorbox{MyColor!35.1309}{as} \colorbox{MyColor!135.8982}{though} \colorbox{MyColor!53.8069}{we} \colorbox{MyColor!66.5958}{were} \colorbox{MyColor!135.8994}{forgotten} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!131.0263}{Waiter} \colorbox{MyColor!66.3253}{was} \colorbox{MyColor!124.8363}{not} \colorbox{MyColor!42.1331}{very} \colorbox{MyColor!134.4877}{attentive} \colorbox{MyColor!33.8659}{and} \colorbox{MyColor!48.367}{they} \colorbox{MyColor!120.9087}{failed} \colorbox{MyColor!35.8341}{to} \colorbox{MyColor!54.0606}{put} \colorbox{MyColor!35.4217}{our} \\ \colorbox{MyColor!42.6813}{order} \colorbox{MyColor!30.6969}{in} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!35.0803}{Ended} \colorbox{MyColor!27.1882}{up} \colorbox{MyColor!32.868}{being} \colorbox{MyColor!32.3232}{there} \colorbox{MyColor!33.8647}{for} \colorbox{MyColor!37.504}{almost} \colorbox{MyColor!39.5842}{2} \colorbox{MyColor!86.4346}{hours} \colorbox{MyColor!35.3435}{because} \colorbox{MyColor!45.0118}{of} \colorbox{MyColor!78.9261}{this} \colorbox{MyColor!10.0}{.} \colorbox{MyColor!75.4464}{good} \colorbox{MyColor!75.467}{was} \colorbox{MyColor!130.332}{amazing} \colorbox{MyColor!40.0523}{and} \colorbox{MyColor!136.3328}{fantastic} \colorbox{MyColor!34.1459}{as} \colorbox{MyColor!39.0689}{far} \\ \colorbox{MyColor!34.6088}{as} \colorbox{MyColor!31.4786}{the} \colorbox{MyColor!56.5627}{brunch} \colorbox{MyColor!65.985}{goes} \colorbox{MyColor!135.2044}{though} \colorbox{MyColor!35.3142}{i} \colorbox{MyColor!136.7223}{would} \colorbox{MyColor!50.2985}{definitely} \colorbox{MyColor!43.8164}{give} \colorbox{MyColor!43.6829}{hash} \colorbox{MyColor!134.8802}{another} \colorbox{MyColor!45.9909}{show} \colorbox{MyColor!37.6619}{because} \colorbox{MyColor!31.6226}{the} \colorbox{MyColor!63.25}{food} \colorbox{MyColor!58.8528}{was} \colorbox{MyColor!46.8313}{delicious} \colorbox{MyColor!10.0}{.} \\ \hline
% \end{tabular}
% \label{tab:viz}
% \end{table*}


% \begin{table}[!t]
% \caption{Table reports the performance of the proposed attention mechanism against various baselines as described in the text. Precision, Recall, F1 Macro(Ma), and F1 Micro(Mi) scores are reported.}
% \label{tab:performance}
% \small
% \begin{tabular}{@{}llllll@{}}
% \toprule
% Datasets & Methods         &  F1  & Accuracy \\ \midrule
%          & HAN-Flat        & 0.91       & 0.915      \\
%          & SA              & 0.864      & 0.876      \\

%          & BiGRU           & 0.898      & 0.905      \\
% News     & CNN             & 0.907      & 0.914      \\
%          & AVG             & 0.905      & 0.91       \\
%          & Our Model       & 0.916      & 0.922      \\
%          & Our Model+ctx   & \textbf{0.919}      & \textbf{0.923}      \\ \midrule
%          & HAN-Flat        &0.879      & 0.971       \\
%          & SA              & 0.765      & 0.942      \\
%          & BiGRU           & 0.459      & 0.867      \\
% Reuters  & CNN             & 0.826      & 0.96       \\
%          & AVG             & 0.221      & 0.795      \\
%          & Our Model       & 0.846      & 0.965      \\
%          & Our Model+ctx   & \textbf{0.905}      & \textbf{0.973}      \\ \midrule
%          & HAN-Flat        & 0.621       & 0.71      \\
%          & SA              & 0.596      & 0.68       \\
%          & BiGRU           & 0.578      & 0.663      \\
% Yelp     & CNN             & 0.62       & 0.693      \\
%          & AVG             & 0.489      & 0.652      \\
%          & Our Model        & 0.607      & 0.697      \\
%          & Our Model+ctx   & \textbf{0.63}       & \textbf{0.716 }     \\ \midrule
%          & HAN-Flat        & 0.608      & 0.655      \\
%          & SA              & 0.591      & 0.638      \\
% Yelp     & BiGRU           & 0.557      & 0.608      \\
% Long     & CNN            & 0.624      & \textbf{0.672}      \\
%          & AVG             & 0.48       & 0.597      \\
%          & Our Model       & 0.612      & 0.653      \\
%          & Our Model+ctx  & \textbf{0.626}      & 0.665      \\ \midrule
%          & HAN-Flat      &	0.895 &	0.895     \\
%          & SA           &	0.831 &	0.831      \\
%          & BiGRU       &	0.876 &	0.876       \\
% IMDB     & CNN        &	0.874 &	0.874     \\
%          & AVG         &	0.874 &	0.874       \\
%          & Our Model      &	0.895 &	0.895     \\
%          & Our Model+ctx &	\textbf{0.9} &	\textbf{0.9}     \\ \midrule
%          & HAN        &    \textbf{0.837}   &  \textbf{0.849}     \\
% MANSA         & HSA     & 0.823 &  0.836   \\
%         & Our Model      &  0.831 &   0.844    \\
%          & Our Model+ctx &  0.823      &      0.841  \\ 
% \end{tabular}
% \end{table}
% ~\ref{tab:performance} indicates the results. We report accuracy for evaluation. 
% All the metrics are reported because for tasks such as event detection individual metrics such as precision or recall might be more helpful. Going forward comparisons are reported based on F1(Micro) scores unless specified.

% \subsection{Effect of Disagreement Regularization}
% In this section we seek to observe the effect of the three disagreement regularizations on the model. As seen from table ~\ref{tab:performance} none of the regularizations seemingly improve model performance of LAMA. However,   

% We plot the disagreement between different attended positions before and after applying the three regularizations. As we can see applying the regularization does increase the disagreement between different attended positions however it doesn't improve the performance. This concurs with observations of similar studies in other NLP tasks ~\citep{li2018multi}.

==> CIKM 2020/sections/rw.tex <==
\section{Related Work} \label{sec:rw}
% \subsection{Sentence Embedding Methods}
% Word embeddings have been shown to learn transferable word representations ~\citep{collobert2011natural,mikolov2013distributed,Pennington2014GloveGV,peters2018deep}.
% Researchers quest for universal embeddings: embeddings that are pre-trained on a large corpus and can be plugged in a variety of downstream task models (sentimental analysis, classification, translation).
% %to automatically improve their performance by incorporating some general word/sentence representations learned on a larger dataset much like in Computer Vision where features obtained from models trained on large datasets such as ImageNet ~\citep{imagenet_cvpr09} can be used for a variety of image classification tasks. 
% Unsupervised representation methods such as averaging a sentence's word vectors gives a strong baseline for many downstream tasks ~\citep{Arora2017ASB}. Another popular unsupervised approach is Skipthoughts ~\citep{Kiros:2015:SV:2969442.2969607} which are equivalent to skip-gram model for word embeddings. QuickThoughts ~\citep{logeswaran2018an} are a faster version of Skipthoughts.
% With the success of InferSent ~\citep{conneau2017word} where a simple model is trained on the SNLI ~\citep{bowman2015large} dataset and learned representations transferred to other tasks supervised sentence embedding methods have started being explored. 
% In learning general purpose distributed sentence representations Subramanian et al. ~\citep{subramanian2018learning}  observe that to be able to generalize over a wide variety of diverse tasks it is essential to capture multiple aspects of a sentence in its representation. They use multi-task learning over several datasets for this task. 
% % The authors thus leverage a one-to-many multi-tasking learning framework to learn a universal sentence embedding by switching between several tasks. 

% In this work, on the contrary, our goal is capture multiple aspects of a sentence required for a specific downstream task without explicit supervision for the aspects.
% \subsection{Distributed representations}
% Distributed memory model introduced in\citep{Le:2014:DRS:3044805.3045025}. The distributed memory model is similar to continuous bag of words model introduced in \citep{NIPS2013_5021} with the only difference that the document vector is treated as additional context along with the other context words.

% Learning vector representations of words and documents is an important research area useful in a variety of natural language processing applications ranging from machine translation~\citep{bilingualMT,sourceTargetMT,alignMT}, question answering`\citep{openQA,metaQA,teachQA} to text retrieval~\citep{wordIR,docIR,queryIR}. Since the introduction of distributed representations approach of words and phrases by Mikolov et al. in~\citep{NIPS2013_5021}, a number of word embedding methods such as~\citep{Levy2014DependencyBasedWE}, \citep{Pennington2014GloveGV}; sentence embedding methods such as <> and document embeddings such as \citep{Le:2014:DRS:3044805.3045025} have been proposed. Most of the these methods are unsupervised and require a large corpus of text to train on. Word embeddings methods try to maximize the word co-occurrence probabilities to assign similar vectors to co-occurring words. Co-occurring words 
% can be words in a contiguous span of text~\citep{NIPS2013_5021} or dependencies of a  word based on the its dependency parse \citep{Levy2014DependencyBasedWE}. To the best of our knowledge our method is the first to do explicit context inference (vocabulary curation) for training the embeddings based on a task. 
% Sentence embedding methods usually are based off of unsupervised word embeddings taking a simple average or a weighted average (cite a simple but hard to beat) of the corresponding word embeddings. \citep{Le:2014:DRS:3044805.3045025} propose a way to jointly train word embeddings and document embeddings.~\citep{Lau2016AnEE} show that doc2vec performs better for longer documents.
% \subsection{Attention Mechanism}
% The practice of applying attention mechanism has a long history particularly in computer vision problems ~\citep{visatt1,visattn2,imCaption}.  Attention mechanism can be of two types. ``Hard'' attention model learns to put attention to only specific parts of the sequences or images ~\citep{revisAttn} whereas, `soft'' attention learns the attention weights over the entire sequence. Gulcehre et al.~\citep{plan} enhance the attention mechanism by incorporating a planning mechanism. Based on the past actions and current observation the model makes a plan of future alignments. Xu et al.~\citep{imCaption} use attention to automatically generate description of images. They have explored both ``soft'' and ``hard'' attention mechanisms. 

% Additionally they enforce constraints so that model put equal attention to every part of the images at the caption generation time. 

% Spearheaded by their success in neural machine translation ~\citep{Bahdanau2014NeuralMT, luong2015effective, neuralAlign, vaswani2017attention} attention mechanisms are used in problems involving sequence to sequence models such as question answering ~\citep{teachQA, seo2016bidirectional, dhingra2016gated} text summarization ~\citep{paulus2017deep, chen2017reading} and visual question answering ~\citep{yu2015combining, yu2017multi}.
% Self-attention ~\citep{lin2017structured} or intra attention ~\citep{han} is used for modeling text for classification tasks. A by-product of self-attention mechanism is visualization of words being attended leading to the explanability of the models.
Spearheaded by their success in neural machine translation ~\citep{neuralAlign,luong2015effective} attention mechanisms are now ubiquitously used in problems such as question answering ~\citep{teachQA, seo2016bidirectional, dhingra2016gated}, text summarization ~\citep{paulus2017deep, chen2017reading}, event extraction ~\citep{Mehta:2019:EDU:3308558.3313659}, and training large language models ~\citep{devlin2018bert,radford2019language}. In sequence modeling, attention mechanisms allow the decoder to learn which part of the sequence it should ``attend'' to based on the input sequence and the output it has generated so far ~\citep{neuralAlign}.

\subsection{Self-Attention}
Self-attention, sometimes called intra-attention is an attention mechanism relating different positions of a single sequence in order to compute a representation of the sequence ~\citep{cheng2016long}. Self-attention has been
used successfully in a variety of tasks including reading comprehension, abstractive summarization, textual entailment and learning task-independent sentence representations ~\citep{cheng2016long, parikh2016decomposable, paulus2017deep,lin2017structured}.
% A special case of attention known as self-attention ~\citep{lin2017structured} or intra-attention ~\citep{han} is used for text classification tasks such as sentiment analysis and natural language inference. 
% A by-product of self-attention mechanism is visualization of words being attended leading to the explainability of the models although some recent work raises questions about use of attention as robust measure for interpretability. 
Traditionally, the above methods have depended on Recurrent Neural Networks(RNNs)~\citep{Hochreiter:1997:LSM:1246443.1246450,Chung2014EmpiricalEO} to model sequential dependencies and attention mechanisms were proposed to alleviate the vanishing gradient problem by establishing shorter connections between the source and target positions. The inherently
sequential nature of RNNs precludes parallelization within training examples which becomes a memory bottleneck for batching across examples. Recently Transformer model was proposed ~\citep{vaswani2017attention} that replaced the dependence on RNNs and relies completely on the self-attention mechanism. In this approach, every position attends to every other position and adjusts its embedding accordingly. However, this dense computation is quadratic in the length of the input and is resource intensive. 
The proposed approach on the contrary leverages RNNs for modeling sequential dependencies and uses a single global query vector for each input word. We show that our approach is computationally more efficient in comparison to encoder of the Transformer model on text classification tasks and exceeds in performance.

\subsection{Multi-Head Attention}
Models have been proposed that compute multiple attention distributions over a single sequence of words. Multi-view networks ~\citep{guo2017end} use a different set of parameters for each view which leads to an increase in the number of parameters.
%with increasing number of views. 
Lin et al. ~\citep{lin2017structured} use the additive attention mechanism, which is a more general approach of computing attention between query and key vectors and modify it to produce multiple attentions to obtain a matrix sentence embedding.
% Both these methods use a special case of additive attention proposed by Bahdanau et al. ~\citep{Bahdanau2014NeuralMT} in the context of neural machine translation.  Luong et al. ~\citep{luong2015effective} simplify additive attention operation by introducing multiplicative attention which is faster to compute. In multiplicative attention, score between two feature vectors is learned using a bilinear projection matrix. Dot product attention ~\citep{luong2015effective} is a special case of multiplicative attention where the score between two features vectors is computed by a simple dot product between them.  Yang et al.
 Scaled dot product attention proposed by Vaswani et. al. ~\citep{vaswani2017attention} is a direct approach and is based on dot product between the query and key vectors. This approach has been shown to be very effective in machine translation ~\citep{vaswani2017attention} and pretraining language models ~\citep{devlin2018bert}. However to compute multiple attention heads different transformation parameters are learned for different heads leading to increased parameters.
% Yang et al. ~\citep{han} use dot product attention to compute the similarity of word hidden representation to a word-level context vector which is learned with the rest of the model. 
In this work, on the other hand, score between the key (context) and the query (word representation) is computed using a bilinear projection matrix followed by an approach inspired by multi-modal low rank bilinear pooling ~\citep{kim2016hadamard} to factorize the matrix into two low rank matrices to compute multiple attention distributions over words.  We find that this is a more parameter efficient way of computing multiple attentions. Contrary to Guo et al. ~\citep{guo2017end} and Vaswani et al. ~\citep{vaswani2017attention} we use matrix factorization to alleviate the problem of increasing parameters with increasing heads and the proposed model performs superior to their approach.

\subsection{Low-Rank Factorization}
Low-rank factorization has been a popular approach to reduce the size of the hidden layers ~\citep{chen2018adaptive,tai2015convolutional}. Recent work has achieved
significant improvements in computational efficiency through factorization tricks ~\citep{shazeer2017outrageously} and conditional
computation ~\citep{kuchaiev2017factorization}. Recently, factorization was also employed at the embedding layer of large pretrained language models such as BERT ~\citep{devlin2018bert} to reduce the model size ~\citep{lan2019albert}. In this work, we employ factorization for unimodal feature fusion for computing attention scores for multiple attention heads. Hadamard product formulation for matrix factorization is used to compactify the multi-head attention layer. This formulation can be viewed as low-rank bilinear pooling for unimodal features based on the corresponding idea of multimodal feature fusion ~\citep{yu2017multi,lin2015bilinear}.
% Multiplicative attention uses a bilinear projection matrix to learn attention score between two feature vectors. Such bilinear pooling has been commonly used for multi-modal feature fusion in visual question answering ~\citep{yu2017multi, lin2015bilinear}, to combine question and paragraph representations in question answering ~\citep{wang2018multi, chen2017reading} or to compute attention between encoder and decoder hidden states in neural machine translation ~\citep{luong2015effective}.


%. It creates an explicit plan of input-output alignments to use at future time-steps, based on its current observation and a summary of its past actions, which it may follow or modify. This enables the model to plan ahead rather than attending to what is relevant primarily at the current generation step.
